Safe and Resilient Multi-vehicle Trajectory Planning Under Adversarial Intruder

Provably safe and scalable multi-vehicle trajectory planning is an important and urgent problem. Hamilton-Jacobi (HJ) reachability is an ideal tool for analyzing such safety-critical systems and has been successfully applied to several small-scale problems. However, a direct application of HJ reachability to multi-vehicle trajectory planning is often intractable due to the "curse of dimensionality." To overcome this problem, the sequential trajectory planning (STP) method, which assigns strict priorities to vehicles, was proposed, STP allows multi-vehicle trajectory planning to be done with a linearly-scaling computation complexity. However, if a vehicle not in the set of STP vehicles enters the system, or even worse, if this vehicle is an adversarial intruder, the previous formulation requires the entire system to perform replanning, an intractable task for large-scale systems. In this paper, we make STP more practical by providing a new algorithm where replanning is only needed only for a fixed number of vehicles, irrespective of the total number of STP vehicles. Moreover, this number is a design parameter, which can be chosen based on the computational resources available during run time. We demonstrate this algorithm in a representative simulation of an urban airspace environment.

==> background/obs_gen3_revised.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Robust Trajectory Tracking (RTT) \label{sec:rtt}}
In this section, we first summarize the basic SPP algorithm in the absence of disturbances and intruder. Robust trajectory tracking method is presented next which account for the disturbances in vehicles' dynamics. The material in this section is taken partially from \cite{Chen15c} and \cite{Bansal2017}. Moreover, only a concise and partial introduction to algorithms is presented here. For more details, interested readers are referred to \cite{Bansal2017}. 

Consider the vehicles' dynamics with disturbances. Here, the dynamics of $\veh_i$ becomes
\begin{equation}
\label{eq:dyn_no_dstb}
\begin{aligned}
\dot\state_i &= \fdyn_i(\state_i, \ctrl_i), t \le \sta_i \\
\ctrl_i &\in \cset_i, \qquad i = 1 \ldots, \N
\end{aligned}
\end{equation}
\noindent where the difference compared to \eqref{eq:dyn} is that the disturbance $d_i$ is no longer a part of the dynamics.

\begin{alg}
\label{alg:basic}
\textbf{Basic SPP algorithm}: Suppose we are given initial conditions $\state_i^0$, vehicle dynamics \eqref{eq:dyn_no_dstb}, target sets $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$. For each $i$ in ascending order starting from $i=1$ (which corresponds to descending order of priority),
\begin{enumerate}
\item determine the total obstacle set $\obsset_i(t)$, given in \eqref{eq:obsseti}. In the case $i=1$, $\obsset_i(t) = \soset_i ~ \forall t$;
\item compute the BRS $\brs_i^\text{basic}(t, \sta_i)$ defined in \eqref{eq:BRS_basic}. The latest departure time $\ldt_i$ is then given by $\arg \sup_t \{\state^0_i \in \brs_i^\text{basic}(t, \sta_i)\}$;
\item determine the trajectory $\state_i(\cdot)$ using vehicle dynamics \eqref{eq:dyn_no_dstb}, with the optimal control  $\ctrl_i^\text{basic}(\cdot)$ given by \eqref{eq:basicOptCtrl};
\item given $\state_i(\cdot)$, compute the induced obstacles $\ioset_k^i(t)$ for each $k>i$. In the absence of disturbances, $\ioset_k^i(t)$ is given by \eqref{eq:ioset}.
\end{enumerate}
\end{alg}

In the basic SPP algorithm, lower priority vehicles know the trajectories of all higher priority vehicles. The region that a lower priority vehicle needs to avoid is thus simply given by the danger zones around these trajectories; however, disturbances and incomplete information significantly complicate the SPP scheme. Committing to exact trajectories is no longer possible, since the disturbance $\dstb_i(\cdot)$ is \textit{a priori} unknown. Thus, the induced obstacles $\ioset_i^j(t)$ are no longer just the danger zones centered around positions. In this section, we provide an overview of the RTT algorithm that can overcome these issues. For simplicity of explanation, we will assume that no static obstacles exist, but method can be generalized even when static obstacles do exist \cite{Bansal2017}. The material in this section is taken partially from \cite{Bansal2017}. Note that even though the theoretical development in Section \ref{sec:intruder} is valid for all three algorithms developed in \cite{Bansal2017} to account for the disturbances, we use RTT algorithm for the simulations in this paper and only present RTT algorithm here. Interested readers are referred to \cite{Bansal2017} for the other two algorithms. 

Even though it is impossible to commit to and track an exact trajectory in the presence of disturbances, it may still be possible to instead \textit{robustly} track a feasible \textit{nominal} trajectory with a bounded error at all times. If this can be done, then the tracking error bound can be used to determine the induced obstacles. Here, computation is done in two phases: the \textit{planning phase} and the \textit{disturbance rejection phase}. 

In the planning phase, a nominal trajectory $\state_{r,j}(\cdot)$ is computed that is feasible in the absence of disturbances. This planning is done for a reduced control set $\cset^p\subset\cset$, as some margin is needed to reject unexpected disturbances while tracking the nominal trajectory.

%In the disturbance rejection phase, we compute a bound on the tracking error.%\MCnote{don't need to explain where error comes bound, imo}%, caused by a vehicle's inability to exactly track the nominal trajectory in the presence of disturbances. 

%It is important to note that the planning phase does not make full use of a vehicle's control authority, as some margin is needed to reject unexpected disturbances while tracking the nominal trajectory. Therefore, in this method, planning is done for a reduced control set $\cset^p\subset\cset$. The resulting trajectory reference will not utilize the vehicle's full control capability; additional maneuverability is available at execution time to counteract external disturbances.

In the disturbance rejection phase, we compute a bound on the tracking error, independently of the nominal trajectory. To compute this error bound, we find a robust controlled-invariant set in the joint state space of the vehicle and a tracking reference that may ``maneuver" arbitrarily in the presence of an unknown bounded disturbance. Taking a worst-case approach, the tracking reference can be viewed as a virtual evader vehicle that is optimally avoiding the actual vehicle to enlarge the tracking error. We therefore can model trajectory tracking as a pursuit-evasion game in which the actual vehicle is playing against the coordinated worst-case action of the virtual vehicle and the disturbance. %In general, this game will be governed by dynamics of the form:

%\begin{equation}
%\label{eq:jdyn} % Joint dynamics
%\begin{aligned}
%\dot{\state_j} &= f_j(t, \state_j, \ctrl_j, \dstb_j), \quad \dot{x_r} =f_j(t,x_r,\ctrl_r,0),\\
%\ctrl_j &\in \cset_j, \ctrl_r\in\cset^\pos_j, d \in \dset_j, \quad t \in [0, T]
%\end{aligned}
%\end{equation}
%where 

Let $\state_j$ and $\state_{r,j}$ denote the states of the actual vehicle $\veh_j$ and the virtual evader, respectively, and define the tracking error $e_j=\state_j-\state_{r,j}$. When the error dynamics are independent of the absolute state as in \eqref{eq:edyn} (and also (7) in \cite{Mitchell05}), we can obtain error dynamics of the form

\begin{equation}
\label{eq:edyn} % Error dynamics
\begin{aligned}
\dot{e_j} &= \fdyn_{e_j}(e_j, \ctrl_j, \ctrl_{r,j},\dstb_j), \\
\ctrl_j &\in \cset_j, \ctrl_{r,j} \in \cset^p_j, \dstb_j \in \dset_j, \quad t \leq 0
\end{aligned}
\end{equation}

To obtain bounds on the tracking error, we first conservatively estimate the error bound around any reference state $\state_{r,j}$, denoted $\errorbound_j$:

\begin{equation} \label{eqn:err}
\errorbound_j = \{e_j: \|\pos_{e_j}\|_2 \le R_{\text{EB}} \}, 
\end{equation}

\noindent where $\pos_{e_j}$ denotes the position coordinates of $e_j$ and $R_{\text{EB}}$ is a design parameter. We next solve a reachability problem with its complement $\errorbound_j^c$, the set of tracking errors violating the error bound, as the target in the space of the error dynamics. From $\errorbound_j^c$, we compute the following BRS:

\begin{equation} \label{eqn:errBound}
\begin{aligned}
\brs^{\text{EB}}_{j}(t, 0) = & \{y: \forall \ctrl_j(\cdot) \in \cfset_j, \exists \ctrl_{r, j}(\cdot) \in \cfset^\pos_j, \exists \dstb_j(\cdot) \in \dfset_i, \\
& e_j(\cdot) \text{ satisfies \eqref{eq:edyn}}, e_j(t) = y, \\
& \exists s \in [t, 0], e_j(s) \in \errorbound_j^c\}, 
\end{aligned}
\end{equation}
where the Hamiltonian to compute the BRS is given by:
\begin{equation}
\begin{aligned}
H^{\text{EB}}_{j}(e_j, \costate) &= \max_{\ctrl_j \in \cset_j} \min_{\ctrl_r \in \cset^\pos_j, \dstb_j \in \dset_j} \costate \cdot \fdyn_{e_j}(e_j, \ctrl_j, \ctrl_{r,j}, \dstb_j).
\end{aligned}
\end{equation}

Letting $t \to -\infty$, we obtain the infinite-horizon control-invariant set $\disckernel_j := \lim_{t \to -\infty} \left( \brs^{\text{EB}}_{j}(t, 0) \right)^c$. If $\disckernel_j$ is nonempty, then the tracking error $e_j$ at flight time is guaranteed to remain within $\disckernel_j \subseteq \errorbound_j$ provided that the vehicle starts inside $\disckernel_j$ and subsequently applies the feedback control law

\begin{equation}
\label{eq:robust_tracking_law}
\tracklaw_j(e_j) = \arg\max_{\ctrl_j \in \cset_j} \min_{\ctrl_r \in\cset^\pos_j, \dstb_j \in \dset_j} \costate \cdot \fdyn_{e_j}(e_j,\ctrl_j,\ctrl_{r, j},\dstb_j).
\end{equation}

%$\disckernel_j$ can be computed in the state space of the tracking error $e_j$ to significantly reduce the problem dimensionality and to produce a feedback control law that also only depends on $e_j$ 
%
%Given an error bound $\errorbound_j(\state_{r,j})$ on the tracking error, we define the target set $\targetset_j$ for this reachability problem to be the set of joint configurations where this bound is violated: $\targetset_j = \{(\state_j, \state_{r,i}): \state_j\not\in\errorbound_j(\state_{r,j})\}$. In this case, the BRS $\brs_j(t)$ represents the set of states from which the vehicle may be driven to violate the tracking error bounds, outside of $\errorbound_j(\state_{r,j})$. $\brs_j(t)$ can be calculated using \eqref{eq:HJIVI} without obstacles, and with the Hamiltonian%With analogous definitions as those in Section \ref{sec:background}, $\brs_j(t)$ can be characterized as the negative region of the solution $V_j$ to a simpler case of \eqref{eq:HJIVI} without obstacles:
%\vspace{-0.2em}
%
%%\begin{small}
%%\begin{equation}
%%\label{eq:HJIVI_track}
%%%\begin{aligned}
%%%\min\big\{&D_t V_j(t, z_j) + \ham_j\left(t, z_j, D_{z_j} V_j\right), l(t,z_j) - V_j(t, z_j)\big\}= 0,\\
%%%&t\in[0,T], \qquad V_j(T, z_j) = l_j(T, z_j) \\
%%\ham_j\left(t, z_j, p\right) = \max_{\ctrl_j \in \cset_j} \min_{\ctrl_r \in\cset^\pos_j} \min_{\dstb_j \in \dset_j} p \cdot \fdyn_{z_j}(t,z_j,\ctrl_j,\ctrl_r,\dstb_j)
%%%\end{aligned}
%%\end{equation}
%%\end{small}
%
%\noindent where for compactness of notation we denote $z_j=(\state_j,x_r)$ and $\fdyn_{z_j}(t,z_j,\ctrl_j,\ctrl_r,\dstb_j) = [f_j(t,\state_j,\ctrl_j,\dstb_j),f_j(t,x_r,\ctrl_r,0)]$. The complement of $\brs_j(0)$ is the maximal robust controlled-invariant set in $\targetset_j^\text{c}$. Letting $T\to\infty$ we obtain the infinite controlled-invariant set, which we denote by $\disckernel_j$. If this set is nonempty, then the tracking error $e_j$ at flight time is guaranteed to remain within $\errorbound_j$ provided that the vehicle starts inside $\disckernel_j$ and subsequently applies the feedback control law implicitly defined in \eqref{eq:HJIVI_track}:
%\begin{equation}\label{eq:robust_tracking_law}
%\tracklaw_j(\state_j,x_r) \in \arg\max_{\ctrl_j \in \cset_j} \min_{\ctrl_r \in\cset^\pos_j, \dstb_j \in \dset_j} p \cdot \fdyn_{z_j}(t,z_j,\ctrl_j,\ctrl_r,\dstb_j).
%\end{equation}

The induced obstacles by each higher-priority vehicle $\veh_j$ can thus be obtained by: 
\begin{equation} 
\label{eqn:rttObs}
\begin{aligned}
\ioset_i^j(t) &=  \{\state_i: \exists y \in \pfrs_j(t), \|\pos_i - y\|_2 \le \rc \} \\
\pfrs_j(t) &= \{\pos_j: \exists \npos_j, (\pos_j, \npos_j) \in \boset_j(t)\} \\
\boset_j(t) &= \disckernel_j  + \state_{r,j}(t),
\end{aligned}
\end{equation}

\noindent where the ``$+$'' in \eqref{eqn:rttObs} denotes the Minkowski sum\footnote{The Minkowski sum of sets $A$ and $B$ is the set of all points that are the sum of any point in $A$ and $B$.}. Intuitively, if $\veh_j$ is tracking $\state_{r,j}(t)$, then it will remain within the error bound $\disckernel_j$ around $\state_{r,j}(t) ~\forall t$. This is precisely the set $\pfrs_j(t)$. The induced obstacles can then be obtained by augmenting a danger zone around this set. Finally, we can obtain the total obstacle set $\obsset_i(t)$ using:
\begin{equation}
\label{eq:obsseti}
\obsset_i(t)  = \soset_i \cup \bigcup_{j=1}^{i-1} \ioset_i^j(t)
\end{equation} 

Since each vehicle $\veh_j$, $j<i$, can only be guaranteed to stay within $\disckernel_j$, we must make sure during the path planning of $\veh_i$ that at any given time, the error bounds of $\veh_i$ and $\veh_j$, $\disckernel_i$ and $\disckernel_j$, do not intersect. This can be done by augmenting the total obstacle set by $\disckernel_i$:%This can be done by choosing the induced obstacle to be the Minkowski sum\footnote{The Minkowski sum of sets $A$ and $B$ is the set of all points that are the sum of any point in $A$ and $B$.} of the error bounds. Thus,

\begin{equation} 
\label{eqn:rttAugObs}
\tilde{\obsset}_i(t) = \obsset_i(t) + \disckernel_i.
\end{equation}

Finally, given $\disckernel_i$, we can guarantee that $\veh_i$ will reach its target $\targetset_i$ if $\disckernel_i \subseteq \targetset_i$; thus, in the path planning phase, we modify $\targetset_i$ to be $\tilde{\targetset}_i := \{\state_i: \disckernel_i + \state_i \subseteq \targetset_i\}$, and compute a BRS, with the control authority $\cset^\pos_i$, that contains the initial state of the vehicle. Mathematically,

\begin{equation}
\label{eq:rttBRS}
\begin{aligned}
\brs_i^\text{rtt}(t, \sta_i) = & \{y: \exists \ctrl_i(\cdot) \in \cfset^p_i, \state_i(\cdot) \text{ satisfies \eqref{eq:dyn_no_dstb}},\\
&\forall s \in [t, \sta_i], \state_i(s) \notin \tilde{\obsset}_i(t), \\
& \exists s \in [t, \sta_i], \state_i(s) \in \tilde{\targetset}_i, \state_i(t) = y\}
\end{aligned}
\end{equation}

The BRS $\brs_i^\text{rtt}(t, \sta_i)$ can be obtained by solving \eqref{eq:HJIVI_BRS} using the Hamiltonian: 
\begin{equation}
\label{eq:RTTham}
\ham_i^\text{rtt}(\state_i, \costate) = \min_{\ctrl_i \in \cset^\pos_i } \costate \cdot \fdyn_i(\state_i, \ctrl_i)
\end{equation}

The corresponding optimal control for reaching $\tilde{\targetset}_i$ is given by:
\begin{equation}
\label{eq:RTTOptCtrl}
\ctrl_i^\text{rtt}(t) = \arg \min_{\ctrl_i \in \cset^\pos_i } \costate \cdot \fdyn_i(\state_i, \ctrl_i).
\end{equation}

The nominal trajectory $\state_{r,i}(\cdot)$ can thus be obtained by using vehicle dynamics in the absence of disturbances
\begin{equation}
\label{eq:dyn_no_dstb}
\begin{aligned}
\dot\state_i &= \fdyn_i(\state_i, \ctrl_i), t \le \sta_i \\
\ctrl_i &\in \cset_i, \qquad i = 1 \ldots, \N,
\end{aligned}
\end{equation}

with the optimal control  $\ctrl_i^\text{rtt}(\cdot)$ given by \eqref{eq:RTTOptCtrl}. From the resulting nominal trajectory $\state_{r,i}(\cdot)$, the overall control policy to reach $\targetset_i$ can be obtained via \eqref{eq:robust_tracking_law}. 

%The robust trajectory tracking method can be summarized as follows:
%\SBnote{Again, we probably don't need to present this algorithm for this paper.}
%\begin{alg}
%\label{alg:rtt}
%\textbf{Robust trajectory tracking algorithm}: Given initial conditions $\state_i^0$, vehicle dynamics \eqref{eq:dyn}, target sets $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$, for each $i$,
%\begin{enumerate}
%\item determine the total obstacle set $\obsset_i(t)$, given in \eqref{eq:obsseti}. In the case $i=1$, $\obsset_i(t) = \soset_i ~ \forall t$;
%\item decide on a reduced control authority $\cset^\pos_i$ for the planning phase, and choose a parameter $R_{\text{EB}}$ to conservatively bound the tracking error;
%\item compute the BRS $\brs^{\text{EB}}_{i}(t, 0)$ using \eqref{eqn:errBound} and make sure that $\disckernel_i \neq \emptyset$. Given $R_{\text{EB}}$, the error bound on the tracking error is given by $\disckernel_i$;
%\item using $\disckernel_i$, determine the augmented obstacle set $\tilde{\obsset}_i(t)$, given in \eqref{eqn:rttAugObs};
%\item compute the BRS $\brs_i^\text{rtt}(t, \sta_i)$ as described in \eqref{eq:rttBRS} using the reduced target set $\tilde{\targetset}_i$, $\tilde{\obsset}_i(t)$ as obstacles, and the control authority $\cset^\pos_i$. The latest departure time $\ldt_i$ is then given by $\arg \sup_t \state^0_i \in \brs_i^\text{rtt}(t, \sta_i)$;
%\item compute the nominal trajectory $\state_{r,i}(\cdot)$ for $\veh_i$ in the absence of disturbances, which can be obtained using the vehicle dynamics in \eqref{eq:dyn_no_dstb} and the optimal control given in \eqref{eq:RTTOptCtrl};
%\item the induced obstacles $\ioset_k^i(t)$ for each $k>i$ can be computed using $\disckernel_i$ and $\state_{r,i}(\cdot)$ via \eqref{eqn:rttObs}.
%\end{enumerate}
%\end{alg}

%\begin{equation}
%\ioset_i^j(t) = \errorbound(0) + \errorbound(\state_{r,j}(t))
%\end{equation}
%now requiring the state (error) to remain in $\errorbound$, so that the target simply becomes $\targetset = \mathbb{R}^n \setminus \errorbound$. In these cases, \eqref{eq:HJIVI_track} is defined on the lower-dimensional state space of relative (error) dynamics (i.e. over $e$ instead of $z$), and the resulting $\disckernel\subset \mathbb{R}^n$ is the discriminating kernel of $\errorbound$. The flight-time tracking error $e$ is then guaranteed to remain within $\errorbound$ provided that the initial error is contained in $\disckernel$ and the vehicle controller applies the optimally robust tracking feedback law \eqref{eq:robust_tracking_law}, which is now of the form $\tracklaw(e)$.

%A price to be paid for using this method is that it imposes more stringent restrictions on the planning. At flight time, the vehicle will apply this robust tracking law around the nominal trajectory instead of the optimal control policy prescribed by the path planner; while constraint satisfaction is guaranteed for the nominal trajectory, this guarantee does not immediately extend to trajectories within the tracking error bound. The natural solution is to ``robustify" the planning by augmenting all obstacles as $\obsset^\errorbound(t) := \obsset(t) - \errorbound$ (with $-$ denoting the Minkowski difference). It then follows directly that if $x_r(t)$ remains clear of $\obsset^\errorbound(t)$ for all $t$, then $x(t)$ remains clear of the original obstacle $\obsset(t)$.

%Based on this, it will be desirable to choose the tracking error bound $\errorbound$ to be as small as possible. The concrete choice of $\errorbound$ will generally correspond to the system designer, since it is specific to the vehicle dynamics, and should always ensure that the resulting discriminating kernel $\disckernel$ (a) is nonempty and (b) contains all expected errors in the initial configuration.

==> intruder_archived_v0/Old_intruder/method1.tex <==
% !TEX root = ../SPP_journal.tex
%Intuitively, the number of vehicles that are affected by an intruder depends on how close the vehicles are to each other. For example, if the vehicles are in a dense configuration, then multiple vehicles might get affected by the intruder simultaneously and hence re-planning is required at a larger scale. In this section, we propose a method that guarantee intruder avoidance while allowing vehicles to be in a dense configuration, but may require a full re-planning of the system after the intruder disappears.     
Suppose some vehicle $\veh_i$ starts avoiding the intruder $\veh_{\intr}$ at some time $t = \tsa$, and stops avoiding at $t = \tea$. When $t < \tsa$, $\veh_i$ must plan its path taking into account the possibility that it may need to avoid an intruder $\veh_\intr$. Since $\veh_i$ may spend a duration of up to $\iat$ performing avoidance, its induced obstacles $\ioset_k^i(t), k>i$ need to be computed in a way that reflects this possibility. The induced obstacles computation is discussed in Section \ref{sec:intruder_iocomp}.

We must also ensure that while avoiding the intruder, $\veh_i$ does not collide with the total obstacle set $\obsset_i(t)$. This requires computing the augmented total obstacle $\tilde\obsset_i(t)$; the computation of $\tilde\obsset_i(t)$ and the controller that guarantees the avoidance of the augmented obstacles are discussed in Section \ref{sec:intruder_aocomp}.

In Section \ref{sec:intruder_avoid}, we describe how $\veh_i$ can guarantee collision avoidance with the intruder.

Finally, when $t > \tea$, $\veh_i$ has already successfully avoided the intruder, but depending on the state it happens to arrive at after avoiding the intruder, it may need to replan its trajectory to reach the target safely. The replanning process is discussed in Section \ref{sec:replan_method1}.

%\begin{itemize}
%\item \textbf{Definitions of 3 different reachable sets (2 additional reachable sets $\frs(\iat, \brs(\ldt, \targetset))$, $\brs(\bar t, \targetset)$ where $\bar t$ is the time vehicle stops avoiding intruder)}.
%\end{itemize}
%
%We are now ready to develop a general theory that takes intruders into account. Our approach to a robust path planning can be summarized in the following steps:
%\begin{itemize}
%\item \textit{Step-1}: First, we compute the set of obstacles induced by the higher priority vehicles for the lower priority vehicles.  
%\item \textit{Step-2}: We then append \textit{all} obstacles (including static ones) by a forward reachable set (FRS) of duration $\iat$. This addendum ensures that if a vehicle starts outside this appended obstacle, then it cannot collide with the obstacle in $\iat$ seconds. Next, we compute a backwards reachable set (BRS) while avoiding these obstacles till it contains the initial state of the vehicle. This set will give us the controller that ensures liveness in the absence of intruders. 
%\item \textit{Step-3}: Compute a $\iat$-step FRS of the BRS computed in Step-2. This FRS is the free flight region that allows a vehicle to avoid any intruder for $\iat$ seconds. We then compute a BRS while avoiding the obstacles induced by the higher priority vehicles (computed in Step-1) \textit{and} that contains the FRS calculated in Step-3. This BRS will give us a controller that guarantee intruder avoidance and liveness. 
%\item \textit{Step-4}: Compute the relative state space wherein we can successfully avoid the intruder for $\iat$ seconds. If a vehicle sense an intruder while it is still outside this region, the above algorithm will ensure safety at all times.  
%\end{itemize}

\subsubsection{Induced Obstacle Computation} \label{sec:intruder_iocomp}
The goal of this section is to compute, for each lower-priority vehicle $\veh_i$, the time-varying obstacles induced by each higher-priority vehicle $\veh_j, j < i$, denoted by $\ioset_i^j(t)$. As before, the total obstacle set $\obsset_i(t)$ can then be obtained using \eqref{eq:obsseti}. To compute the obstacle that $\veh_i$ needs to avoid at time $t$, it is sufficient to consider the scenarios where $\tsa \in [t-\iat, t]$. This is because if $\tsa < t - \iat$, then the SPP vehicles will already be in the replanning phase at time $t$ and hence cannot be in conflict. 

Depending on the information known to a lower-priority vehicle $\veh_i$ about $\veh_j$'s control strategy, we can use one of the three methods described in Section \ref{sec:incomp} to compute the ``base" obstacles $\boset_j(t)$ , the obstacles that would have been induced by $\veh_j$ in the absence of an intruder. The base obstacles are respectively given by \eqref{eqn:ccObs_help2}, \eqref{eqn:lrcObs3} and \eqref{eqn:rttObs} for centralized control, least restrictive control and robust trajectory tracking.  

The induced obstacles, $\ioset_i^j(t)$, are then given by the states that $\veh_j$ can reach while avoiding the intruder, starting from some state in $\boset_j(\tsa), \tsa \in [t-\iat, t]$. These states can be obtained by computing a FRS from the base obstacles.
\begin{equation} \label{eq:FRS_intObs1}
\begin{aligned}
\frs_{j}^{\mathcal{O}}(0, \tau) = & \{y: \exists \ctrl_j(\cdot) \in \cfset_j, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(0) \in \boset_j(t-\tau), \\
& \state_j(\iat) = y\}.
\end{aligned}
\end{equation}
$\frs_{j}^{\mathcal{O}}(0, \tau)$ represents the set of all possible states that $\veh_j$ can reach after a duration of $\tau$ starting from inside $\boset_j(t-\tau)$. This FRS can be obtained by solving the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:
\begin{equation}
\ham_{j}^{\mathcal{O}}(\state_j, \costate) = \max_{\ctrl_j \in \cset_j} \max_{\dstb_j \in \dset_j} \costate \cdot f_j (\state_j, \ctrl_j, \dstb_j) \label{intobs2}.
\end{equation} 
Since $\tau \in [0, \iat]$, the induced obstacles can be obtained as:
\begin{equation} \label{eq:intObs}
\begin{aligned}
\ioset_i^j(t) & = \{\state_i: \exists y \in \pfrs_j(t), \|\pos_i - y\|_2 \le \rc \}\\
\pfrs_j(t) & = \{p_j: \exists \npos_j, (p_j, \npos_j) \in \bigcup_{\tau \in [0, \iat]} \frs_{j}^{\mathcal{O}}(0, \tau) \}
\end{aligned}
\end{equation}

Note that by the definition of base obstacles, $\boset_j(t+\tau_2) \subseteq \frs_{j}^{\text{BO}}(0, \tau_2-\tau_1) ~\forall t, \tau_2 > \tau_1$, where $\frs_{j}^{\text{BO}}(0, \tau_2-\tau_1)$ denotes the FRS of $\boset_j(t+\tau_1)$ computed for a duration of $\tau_2-\tau_1$. Therefore, we have that $\frs_{j}^{\mathcal{O}}(0, \tau) \subset \frs_{j}^{\mathcal{O}}(0, \iat) ~\forall \tau \in [0, \iat)$. Thus, $\pfrs_j(t)$ in \eqref{eq:intObs} can be equivalently written as:
\begin{equation} \label{eq:intObs_help1}
\pfrs_j(t) = \{p_j: \exists \npos_j, (p_j, \npos_j) \in \frs_{j}^{\mathcal{O}}(0, \iat) \}.
\end{equation}

%
%Since there are no moving vehicle obstacles for the highest priority vehicle, $\obsset_1(t) = \soset$. 
%
%Computation of these base obstacles would requires information of a corresponding ``base" BRS of $\veh_j$; the process for computing this set is outlined in Step 2. In this section, we assume that the sequence of base obstacles, $\boset_i^j(t)$, is known. Given $\boset_i^j(t)$, we now show how to compute the obstacle set $\obsset_i(t)$. The induced obstacles are given by the states a vehicle can reach while avoiding the intruder, on top of the base obstacles. 

\subsubsection{Augmented Obstacle Computation} \label{sec:intruder_aocomp}
We next need to ensure that $\veh_i$ doesn't collide with the obstacles $\obsset_i(\cdot)$ computed in Section \ref{sec:intruder_iocomp} even when it is avoiding the intruder. In particular, we can compute a region around the obstacles $\obsset_i(\cdot)$ such that for all disturbances, $\veh_i$ can avoid colliding with obstacles for $\iat$ seconds regardless of its avoidance control, if $\veh_i$ starts outside this region. Augmenting $\obsset_i(\cdot)$ with this region gives us the augmented obstacles, $\tilde\obsset_i(\cdot)$, that can then be used during the path planning of $\veh_i$ to ensure collision avoidance with $\obsset_i(\cdot)$.  

Suppose that the intruder appears in the system at time $\tsa = t - \iat + \tau, \tau \in [0, \iat]$. In this case, we need to ensure that $\veh_i$ does not collide with the obstacle $\obsset_i(t + \tau)$ at time $t + \tau$, regardless of its control $\ctrl_i(s)$ and disturbance $\dstb_i(s)$ for the time interval $s \in [\tsa, t + \tau]$. It is, therefore, sufficient to avoid the $\tau$-horizon BRS of $\obsset_i(t + \tau)$ at time $t$. This argument applies for all $\tau \in [0, \iat]$. Mathematically,

%\begin{equation} \label{eqn:inducedobs}
%\tilde\obsset_i(t) = \bigcup_{\tau \in [0, \iat]} \brs_{\mathcal{G}}(\tau, \obsset_i(t+\tau), \emptyset, \ham_{\mathcal{G}})
%\end{equation}
%where $\brs_{\mathcal{G}}(\tau, \obsset_i(t+\tau), \emptyset, \ham_{\mathcal{G}})$ represents BRS of $\obsset_i(t+\tau)$ computed backwards for $\tau$ seconds. The Hamiltonian 
%$\ham_{\mathcal{G}}$ is given by:
\begin{equation} \label{eqn:inducedobs}
\tilde\obsset_i(t) = \bigcup_{\tau \in [0, \iat]} \brs^{\mathcal{G}}_{i}(0, \tau)
\end{equation}
where $\brs^{\mathcal{G}}_{i}(0, \tau)$ represents BRS of $\obsset_i(t+\tau)$ computed backwards for $\tau$ seconds. Formally, 
\begin{equation} \label{eqn:inducedobs_help1}
\begin{aligned}
\brs^{\mathcal{G}}_{i}(0, \tau) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(0) = y, \\
& \exists s \in [0, \tau], \state_i(s) \in \obsset_i(t+\tau)\}.
\end{aligned}
\end{equation}

The Hamiltonian $\ham^{\mathcal{G}}_{i}$ to compute $\brs^{\mathcal{G}}_{i}(\cdot)$ is given by:
\begin{equation} \label{eqn:BRS_obsham}
\ham^{\mathcal{G}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

\begin{remark}
Note that if we use the robust trajectory tracking method to compute the base obstacles, we need to augment the obstacles in \eqref{eqn:inducedobs} by the error bound of $\veh_i$, $\disckernel_i$, as discussed in section \ref{sec:rtt}.
\end{remark}

Finally, we compute a BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ for path planning that contains the initial state of $\veh_i$ while avoiding these augmented obstacles:
\begin{equation} \label{eqn:intrBRS1}
\begin{aligned}
\brs^{\text{AO}}_{i}(t, \sta_i) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \forall \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \forall s \in [t, \sta_i], \state_i(s) \notin \tilde\obsset_i(s), \\
& \exists s \in [t, \sta_i], \state_i(s) \in \targetset_i, \state_i(t) = y \}.
\end{aligned}
\end{equation}
The Hamiltonian $\ham^{\text{AO}}_{i}$ to compute BRS in \eqref{eqn:intrBRS1} is given by:
\begin{equation} \label{eqn:BRSham}
\ham^{\text{AO}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

Note that $\brs^{\text{AO}}_{i}(\cdot)$ ensures liveness for $\veh_i$ in the absence of intruder. The liveness controller is given by:
\begin{equation}
{\ctrl^{\text{AO}}_{i}} = \arg \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}
Moreover, if $\veh_i$ starts within $\brs^{\text{AO}}_{i}$, it is guaranteed to avoid collision for a duration of $\iat$, starting at any $\tsa < \sta_i$, irrespective of the control and disturbance applied during this time period. 

\subsubsection{Optimal Avoidance Controller} \label{sec:intruder_avoid}
First, we define relative dynamics of the intruder $\veh_{\intr}$ with state $\state_\intr$ with respect to $\veh_i$ with state $\state_i$.

\begin{equation}
\label{eq:reldyn}
\begin{aligned}
\state_{\intr, i} &= \state_\intr - \state_i \\
\dot \state_{\intr, i} &= f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}

Given the relative dynamics, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_i$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. This set of states is given by the backwards reachable set $\brs^{\text{CA}}(t, \iat),~ t \in [0, \iat]$:%(\iat, \targetset_\text{CA}, \obsset_\text{CA}, H_\text{CA})$, with

\begin{equation} \label{eqn:optAvoid}
\begin{aligned}
\brs^{\text{CA}}_{i}(t, \iat) = & \{y: \forall \ctrl_i(\cdot) \in \cfset_i, \exists \ctrl_\intr(\cdot) \in \cfset_\intr, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \exists \dstb_\intr(\cdot) \in \dfset_\intr, \state_{\intr, i}(\cdot) \text{ satisfies \eqref{eq:reldyn}},\\
& \exists s \in [t, \iat], \state_{\intr, i}(s) \in \targetset^{\text{CA}}_{i}, \state_{\intr, i}(t) = y\},
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\targetset^{\text{CA}}_{i} &= \{\state_{\intr, i}: \|\pos_{\intr, i}\|_2 \le \rc\} \\
H^{\text{CA}}_{i}(\state_{\intr, i}, \costate) &= \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{aligned}
\end{equation}

Once the value function $\valfunc^{\text{CA}}_{i}(\cdot)$ is computed, the optimal avoidance control ${\ctrl^{\text{CA}}_{i}}$ can be obtained as:
\begin{equation} \label{eqn:optAvoidCtrl}
{\ctrl^{\text{CA}}_{i}} = \arg \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{equation}

Under normal circumstances when the intruder $\veh_{\intr}$ is far away, we have $\valfunc^{\text{CA}}_{i}(0, \state_{\intr, i}(t)) > 0$; as $\veh_{\intr}$ gets closer to $\veh_i$, $\valfunc^{\text{CA}}_{i}(0, \state_{\intr, i}(t))$ decreases. If $\veh_i$ applies the control ${\ctrl^{\text{CA}}_{i}}$ when $\valfunc^{\text{CA}}_{i}(0, \state_{\intr, i}(t)) = 0$, then collision avoidance between $\veh_i$ and $\veh_{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

In addition, obstacle augmentation \eqref{eqn:inducedobs} ensures that $\veh_i$ does not collide with $\obsset_i(\cdot)$ during the avoidance maneuver. %Therefore, applying $\ctrl_I^A$ for a duration of $\iat$ is still guaranteed to keep $\veh_i$ safe from all obstacles, and hence safe from collision with respect to all other vehicles $\veh_j, j \neq i$.
The overall control policy for avoiding the intruder and collision with other vehicles is thus given by:
\begin{equation*}
{\ctrl^{\text{A}}_{i}}(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{AO}}_{i}}(t) & t \leq \tsa\\
{\ctrl^{\text{CA}}_{i}}(t) & \tsa\leq t \leq \tea
\end{array}
\right.
\end{equation*}

\subsubsection{Replanning after intruder avoidance\label{sec:replan_method1}} 
After the intruder disappears, liveness controllers which ensure that the vehicles reach their destinations can be obtained by solving a SPP problem as described in Section \ref{sec:incomp}, where the starting states of the vehicles are now given by the states they end up in, denoted $\tilde{\state}_j^0$, after avoiding the intruder. Let the optimal control policy corresponding to this liveness controller be denoted ${\ctrl^{\text{L}}_{i}}(t)$. The overall control policy that ensures intruder avoidance, collision avoidance with other vehicles, and successful transition to the destination is given by:

\begin{equation*}
\ctrl_i^*(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{A}}_{i}}(t) & t \leq \tea\\
{\ctrl^{\text{L}}_{i}}(t) & t > \tea
\end{array}
\right.
\end{equation*}

Note that in order to replan using a SPP method, we need to determine feasible $\sta$s for all vehicles. This can be done by computing an FRS:
\begin{equation} \label{eq:replanFRS}
\begin{aligned} 
\frs_j^{\text{RP}}(\tea, t) = & \{y \in \R^{n_j}: \exists \ctrl_j(\cdot) \in \cfset_j, \forall \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(\tea) = \tilde{\state}_j^0, \\
& \state_j(t) = y, \forall s \in [\tea, t], \state_j(s) \notin \obsset_j^{\text{RP}}(s) \},
\end{aligned}
\end{equation}
where $\tilde{\state}_j^0$ represents the state of $\veh_j$ at $t = \tea$; $\obsset_j^{\text{RP}}(\cdot)$ takes into account the fact that $\veh_j$ needs to avoid higher-priority vehicles $\veh_k, k<j$ and is given by:
\begin{equation} 
\obsset_j^{\text{RP}}(t) = \bigcup_{k<j} \frs_k^{\text{RP}}(\tea, t), ~~~t > \tea.
\end{equation}

The FRS in \eqref{eq:replanFRS} can be obtained by solving the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:
\begin{equation}
\ham_j^{\text{RP}}(\state_j, \costate) = \max_{\ctrl_j \in \cset_j} \min_{\dstb_j \in \dset_j} \costate \cdot f_j (\state_j, \ctrl_j, \dstb_j). 
\end{equation} 
The new $\sta$ of $\veh_j$ is now given by the earliest time at which $\frs_j^{\text{RP}}(\tea, t)$ intersects the target set $\targetset_j$, $\sta_j := \arg \inf_t \{ \frs_j^{\text{RP}}(\tea, t) \cap \targetset_j \neq \emptyset \}$. Intuitively, this means that there exists a control policy which will steer the vehicle to its destination by that time, despite the worst case disturbance it might experience.

\begin{remark}
Note that we only need to replan the trajectories of the vehicles that are affected by the intruder. In particular, if $\valfunc^{\text{CA}}(0, \state_{\intr, i}(t)) > 0$ during the entire duration $t \in [\tsa, \tea]$ for a vehicle, then the vehicle would need not to apply any avoidance control, and hence a replanning would not be required for this vehicle. 
\end{remark}

\begin{remark}
In general, an intruder can be present in the system for much longer than $\iat$, as long as it is not affecting the SPP vehicles. $\underbar{t}$ thus really corresponds to the time an intruder starts affecting a SPP vehicle.
\end{remark}

\begin{remark}
Note that even though we have presented the analysis for one intruder, the proposed method can handle multiple intruders as long as only one intruder is present \textit{at any given time}. 
\end{remark}

We conclude this section with the overall algorithm to successfully avoid an intruder for a duration of $\iat$: 
\begin{alg}
\label{alg:intruder}
\textbf{Intruder Avoidance algorithm (offline-planning)}: Given initial conditions $\state_i^0$, vehicle dynamics \eqref{eq:dyn}, intruder dynamics in Assumption \ref{as:dynKnown}, target sets $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$, for each $i$:
\begin{enumerate}
\item Determine the total obstacle set $\obsset_i(t)$, given in \eqref{eq:obsseti}. In the case $i=1$, $\obsset_i(t) = \soset_i ~ \forall t$.
\item Compute the augmented obstacle set $\tilde\obsset_i(t)$ given by \eqref{eqn:inducedobs}, where $\brs^{\mathcal{G}}_{i}(0, \tau)$ is given by \eqref{eqn:inducedobs_help1}.
\item Given $\tilde\obsset_i(t)$, compute the BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ defined in \eqref{eqn:intrBRS1}.
\item The optimal control to avoid the intruder can be obtained by computing $\brs^{\text{CA}}_{i}(t, \iat)$ in \eqref{eqn:optAvoid} and using \eqref{eqn:optAvoidCtrl}. 
\item The induced obstacles $\ioset_k^i(t)$ for each $k>i$ can be computed using \eqref{eq:intObs}.
\end{enumerate}

\textbf{Intruder Avoidance algorithm (online-planning)}:
\begin{enumerate}
\item Compute $\frs_i^{\text{RP}}(\tea, t)$ using $\eqref{eq:replanFRS}$. The new $\sta_i$ for $\veh_i$ is given by $\arg \inf_t \{ \frs_j^{\text{RP}}(\tea, t) \cap \targetset_j \neq \emptyset \}$.
\item Given $\sta_i$, $\tilde{\state}_i^0$, vehicle dynamics \eqref{eq:dyn}, target set $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$, use any of the three SPP methods discussed in Section \ref{sec:incomp} for replanning. 
\end{enumerate}
\end{alg}

==> intruder_archived_v0/Old_intruder/step1.tex <==
% !TEX root = ../SPP_journal.tex
\subsection{Step 1: Induced Obstacle Computation \label{sec:intruder_iocomp}}
The goal of this section is to compute, for each lower priority vehicle $\veh{i}$, the time-varying obstacle induced by each higher priority vehicle $\veh{j}, j < i$, denoted by $\ioset_i^j(t)$. As before, once $\ioset_i^j(t)$ is computed, one can then solve \eqref{eq:HJIVI_i} with the union of all obstacles induced by higher priority vehicles as the total obstacle set $\obsset_i(t)$. 

Note that since there are no moving vehicle obstacles for the highest priority vehicle, $\obsset_1(t) = \soset$. To compute the obstacle set $\ioset_i^j(t)$ where $i> 1$, we first compute the ``base" obstacles using any of the three methods outlined in Section \ref{sec:incomp}. Base obstacles correspond to the states which a vehicle can reach when it is not avoiding an intruder. Computation of these base obstacles would requires information of a corresponding ``base" BRS of $\veh{j}$; the process for computing this set is outlined in Step 2. In this section, we assume that the sequence of base obstacles, $\boset_i^j(t)$, is known. Given $\boset_i^j(t)$, we now show how to compute the obstacle set $\obsset_i(t)$. 

The induced obstacles are given by the states a vehicle can reach while avoiding the intruder, on top of the base obstacles. Since a vehicle avoids the intruder for a maximum of $\iat$, these states can be given by the $\iat$-horizon FRS of the base obstacle. Regardless of what control is used by $\veh{j}$ for avoidance, it still remains within the FRS $\ioset_i^j(t) := \frs_{\mathcal{O}}(\iat, \boset_i^j(t-\iat), \emptyset, \ham_{\mathcal{O}})$, which is the set of all possible states that $\veh{j}$ can reach after a duration of $\iat$ starting from inside $\boset_i^j(t-\iat)$. Here, the Hamiltonian is given by

\begin{equation}
\ham_{\mathcal{O}}(\state_j, p) = \min_{\ctrl_j} \min_{\dstb_j} p \cdot f_j (\state_j, \ctrl_j, \dstb_j)
\end{equation}


==> intruder_archived_v0/Old_intruder/step2.tex <==
% !TEX root = ../SPP_journal.tex
\subsection{Step 2: Augmented Obstacle Computation \label{sec:intruder_aocomp}}
The goal of this section is to compute a region around the obstacles $\obsset_i(\cdot)$ such that for all disturbances, $\veh{i}$ can avoid colliding with any obstacle for $\iat$ seconds if $\veh{i}$ starts outside this region. The utility of computing such a region will become clearer in Step 3. 

We let $\tilde\obsset_i(t)$ denote the region, which can be thought of as a set of augmented obstacles. To ensure that a vehicle does not hit the obstacle $\obsset_i(t_1 + t')$ at time $t = t_1 + t'$ starting at $t = t_1$, even when it applies any control for the next $t'$ seconds, it suffices to avoid the $t'$-horizon BRS of $\obsset_i(t_1 + t')$. This argument applies for all obstacles to appear in the next $\iat$ seconds to ensure safety under any controller and disturbance for the next $\iat$ seconds. Mathematically,

\begin{equation} \label{eqn:inducedobs}
\tilde\obsset_i(t) = \bigcup_{\tau \in [0, \iat]} \brs_{\mathcal{G}}(\tau, \obsset_i(t+\tau), \emptyset, \ham_{\mathcal{G}})
\end{equation}
where $\brs_{\mathcal{G}}(\tau, \obsset_i(t+\tau), \emptyset, \ham_{\mathcal{G}})$ represents BRS of $\obsset_i(t+\tau)$ computed backwards for $\tau$ seconds. The Hamiltonian 
$\ham_{\mathcal{G}}$ is given by:

\begin{equation} \label{eqn:BRSham}
\ham_{\mathcal{G}}(\state_i, p) = \min_{\ctrl_i} \min_{\dstb_i} p \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

Finally, we compute a BRS that contains the initial state of $\veh{i}$ while these augmented obstacles, $\brs_\text{AO}(t, \targetset_i, \bar\obsset_i, \ham_\text{AO})$, where $\ham_\text{AO} = \ham_{\mathcal{G}}$ (\textbf{Somil}: this is not correct. Disturbance should maximize the Hamiltonian for this BRS.) Note that this BRS ensures liveness for $\veh{i}$ in the absence of intruder. Moroever, if we start from $\brs_\text{AO}$, we are guaranteed to avoid collision for $\iat$ seconds, irrespective of control and disturbance applied. 

==> intruder_archived_v0/Old_intruder/step3.tex <==
% !TEX root = ../SPP_journal.tex
\subsection{Step 3: Intruder Avoidance \label{sec:intruder_after}}
\MCnote{This section doesn't seem like intruder avoidance}
Under Assumption \ref{as:avoidOnce}, a vehicle $\veh{i}$ does not need to avoid an intruder more than once. Thus, after performing an avoidance maneuver, $\veh{i}$ can simply resume moving towards its destination given by $\targetset_i$ while avoiding the (un-augmented) obstacles $\obsset_i(t)$ in \eqref{eq:obsseti}\MCnote{Add equation reference}. The optimal controller for this task is obtained from the BRS $\brs_\text{L}(t, \targetset_i, \obsset_i, \ham_\text{liveness}$) given in Section \ref{sec:basic}.

\subsubsection{Time-to-reach bound after intruder avoidance}
Before avoiding the intruder $\veh{\intr}$, vehicle $\veh{i}$ uses the controller $\ctrl^*_\text{AO}(t, \state_i; \targetset_i, \tilde\obsset_i, \ham_\text{AO})$, which by construction keeps its state $\state_i$ within the BRS $\brs_\text{AO}(t, \targetset_i, \tilde\obsset_i, \ham_\text{AO})$. When $\veh{\intr}$ interferes, $\veh{i}$ is forced to perform an avoidance maneuver for a duration of up to $\iat$ in order to avoid collisions. 

Regardless of what control is used for avoidance, $\veh{i}$ still remains within the FRS 

\begin{equation}
\frs_\text{APS}(\iat, \brs(t, \targetset_i, \obsset_i, \ham_\text{nom}), \emptyset, \ham_\text{APS}), 
\end{equation}

\noindent which is the set of all possible states that $\veh{i}$ can reach starting from inside $\brs_\text{AO}(t)$. Here, the Hamiltonian is given by

\begin{equation}
\ham_\text{APS}(\state_i, p) = \min_{\ctrl_i} \min_{\dstb_i} p \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

Let $\wcttr$ be the smallest time horizon for the BRS $\brs(\wcttr, \targetset_i, \obsset_i, \ham_\text{L})$ such that it contains $\frs(\iat, \brs(t, \targetset_i, \obsset_i, \ham_\text{nom}), \emptyset, \ham_\text{APS})$ entirely. Then, $\wcttr$ would be an upper bound on the time that $\veh{i}$ needs to safely arrive at $\targetset_i$ after avoiding the intruder $\veh{\intr}$.

==> intruder_archived_v0/Old_intruder/step4.tex <==
% !TEX root = ../SPP_journal.tex
\subsection{Step 4: Optimal Avoidance Controller \label{sec:intruder_avoid}}
First, we define relative coordinates of the intruder $\veh{\intr}$ with state $\state_\intr$ with respect to $\veh{i}$ with state $\state_i$.

\begin{equation}
\label{eq:reldyn}
\begin{aligned}
\state_r &= \state_\intr - \state_i \\
\dot \state_r &= f_r(\state_r, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}

Given the relative dynamics, we compute the set of states from which the joint states of $\veh{\intr}$ and $\veh{i}$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh{i}$ to avoid $\veh{\intr}$. Under the relative dynamics \eqref{eq:reldyn}, this set of states is given by the backwards reachable set $\brs(\iat, \targetset_\text{CA}, \obsset_\text{CA}, H_\text{CA})$, with

\begin{equation}
\begin{aligned}
\targetset_\text{CA} &= \{\state_r: \|\pos_r\|_2 \le \rc\} \\
\obsset_\text{CA} &= \emptyset \\
H_\text{CA}(\state_r, p) &= \max_{\ctrl_i} \min_{\ctrl_\intr} p \cdot f_r(\state_r, \ctrl_i, \ctrl_\intr)
\end{aligned}
\end{equation}

Once the value function $\valfunc_\text{CA}(t, \state_r)$ representing $\brs_\text{CA}(\iat, \targetset_\text{CA}, \obsset_\text{CA}, H_\text{CA})$ is computed, the optimal avoidance control $\ctrl^*_\text{CA}$ can be derived from \eqref{eq:opt_ctrl}.

Under normal circumstances when the intruder $\veh{\intr}$ is far away, we have $\valfunc_\text{CA}(\iat, \state_r) > 0$; as the $\veh{\intr}$ gets closer to $\veh{i}$, $\valfunc_\text{CA}(\iat, \state_r)$ decreases. If $\veh{i}$ applies the control $\ctrl^*_\text{CA}$ when $\valfunc_\text{CA}(\iat, \state_r) = 0$, then collision avoidance between $\veh{i}$ and $\veh{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

In addition, under Assumption \ref{as:avoidOnce}, we have $\state_i \in \brs(\bar t, \targetset_i, \tilde\obsset(t))$. Therefore, applying $\ctrl_I^A$ for a duration of $\iat$ is still guaranteed to keep $\veh{i}$ safe from all obstacles, and hence safe from collision with respect to all other vehicles $\veh{j}, j \neq i$.

==> intruder_archived_v0/avoid_control.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Optimal Avoidance Controller} \label{sec:intruder_avoid}
To compute the optimal avoidance control for $\veh_i$ in presence of $\veh_{\intr}$, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_i$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. 

We define relative dynamics of the intruder $\veh_{\intr}$ with state $\state_\intr$ with respect to $\veh_i$ with state $\state_i$:
\begin{equation}
\label{eq:reldyn}
\begin{aligned}
\state_{\intr, i} &= \state_\intr - \state_i \\
\dot \state_{\intr, i} &= f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}
Given the relative dynamics, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_{i}$ can enter danger zone $\dz_{i\intr}$ in a duration of $\iat$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. Under the relative dynamics \eqref{eq:reldyn}, this set of states is given by the backwards reachable set $\brs^{\text{A}}_i(\tau, \iat),~ \tau \in [0, \iat]$:

\begin{equation} \label{eqn:avoidBRS}
\begin{aligned}
\brs^{\text{A}}_{i}(\tau, \iat) = & \{y: \forall \ctrl_i(\cdot) \in \cfset_i, \exists \ctrl_\intr(\cdot) \in \cfset_\intr, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \exists \dstb_\intr(\cdot) \in \dfset_\intr, \state_{\intr, i}(\cdot) \text{ satisfies \eqref{eq:reldyn}},\\
& \exists s \in [\tau, \iat], \state_{\intr, i}(s) \in \targetset^{\text{A}}_{i}, \state_{\intr, i}(\tau) = y\},
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\targetset^{\text{A}}_{i} = & \{\state_{\intr, i}: \|\pos_{\intr, i}\|_2 \le \rc\} \\
H^{\text{A}}_{i}(\state_{\intr, i}, \costate) = & \max_{\ctrl_i \in \cset_i} \left( \right.\\
&\left. \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{aligned}
\end{equation}

We refer to $\brs^{\text{A}}_i(\tau, \iat)$ as \textit{avoid region} hereon. Once the value function $\valfunc^{\text{A}}_{i}(\cdot)$ is computed, the optimal avoidance control ${\ctrl^{\text{A}}_{i}}$ can be obtained as:
\begin{equation} \label{eqn:optAvoidCtrl}
{\ctrl^{\text{A}}_{i}} = \arg \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{equation}

Let $\partial \brs^{\text{A}}_{i}(\cdot, \iat)$ denotes the boundary of the set $\brs^{\text{A}}_{i}(\cdot, \iat)$. The interpretation of $\brs^{\text{A}}_{i}(\tau, \iat)$ is that if $\state_{\intr, i}(t) \in \partial \brs^{\text{A}}_{i}(\tau, \iat)$, then $\veh_i$ can successfully avoid the intruder for a duration of $(\iat - \tau)$ using the optimal avoidance control in \eqref{eqn:optAvoidCtrl}. In the worst case, $\veh_i$ might need to avoid the intruder for a duration of $\iat$; thus, we must have that  
$\state_{\intr, i}(\tsa) \in \left(\brs^{\text{A}}_{i}(0, \iat)\right)^C$. Equivalently, every SPP vehicle should be able to detect the intruder at a distance of $\dsen$, where
\begin{equation} \label{eqn:sen_distance}
\dsen = \max\{ \|a\|: a \in \brs^{\text{A}}_{i}(0, \iat) \}.
\end{equation} 
Hereon, we assume that every SPP vehicle can detect the intruder at a distance of $\dsen$.

%Under normal circumstances when the intruder $\veh_{\intr}$ is far away, we have $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) > 0$; as $\veh_{\intr}$ gets closer to $\veh_i$, $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t))$ decreases. If $\veh_i$ applies the control ${\ctrl^{\text{S}}_{i}}$ when $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) = 0$, then collision avoidance between $\veh_i$ and $\veh_{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

==> intruder_archived_v0/buffRegion.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Buffer Region} \label{sec:buffRegion}
In section \ref{sec:sepRegion}, we computed sets $\sep_j(\cdot)$ such that $\veh_j$ avoids the intruder only if $\state_{\intr}(t) \in \sep_j(t)$. But to ensure that atmost $\nva$ vehicles need to replan their trajectories after the intruder disappears, we need to make sure that the intruder can cause atmost $\nva$ vehicles to deviate from their planned trajectories. Equivalently, we want to ensure that atmost $\nva$ vehicles need to avoid the intruder, that is $\veh_{\intr}$ enters the separation regions of atmost $\nva$ vehicles during a duration of $\iat$.

Intuitively, we want to make sure that at any given time the separation regions of any two vehicles are far enough from each other (that is, there is a ``buffer" region between two separation regions) such that it will take at least $\brd := \iat / \nva$ time for the intruder to go from the separation region of one vehicle to that of the other vehicle. This means that there is a ``buffer" time interval of $\brd$ between any $t_1$, $t_2 \in [\tsa, \tea]$ where $\veh_{\intr}$ is in the separation regions of two different vehicles at $t_1$ and $t_2$, e.g. $\state_{\intr}(t_1) \in \sep_j(t)$ and $\state_{\intr}(t_2) \in \sep_i(t)$, $i \neq j$. Thus, in the worst case, the intruder can force atmost $\nva$ vehicles to apply avoidance maneuver during a duration of $\iat$. 

We next focus on computing the buffer region between any two vehicles $\veh_j$ and $\veh_i$, $j < i$. We first make the following observation:
\begin{observation} \label{obs1_buffReg}
Without loss of generality, we can assume that the intruder appears at the boundary of the separation region of a SPP vehicle at $t = \tsa$, e.g. $\state_{\intr}^0 \in \partial \sep_m(\tsa)$ for some $m \in \{1, \ldots, N\}$, where $\partial \sep_m(\tsa)$ denotes the boundary of $\sep_m(\tsa)$. Otherwise, any vehicle need not account for the intruder until it reaches the boundary of the separation region of a SPP vehicle. 
\end{observation}
Therefore, to compute the buffer region between $\veh_j$ and $\veh_i$, it is sufficient to consider the following two cases:     
\subsubsection{Case1- $\state_{\intr}^0 \in \sep_j(\tsa)$} \label{sec:buffCase1}
Given the relative dynamics $\state_{i, \intr}$ in \eqref{eq:reldyn}, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_{i}$ can enter danger zone $\dz_{i\intr}$ within a duration of $\brd$ when both $\veh_{i}$ and $\veh_{\intr}$ are using \textit{optimal control to collide} with each other. This set of states is given by the backwards reachable set $\brs^{\text{B}}_i(\tau, \brd)$:

\begin{equation} \label{eqn:buffBRS}
\begin{aligned}
\brs^{\text{B}}_{i}(t, \brd) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \ctrl_\intr(\cdot) \in \cfset_\intr, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \exists \dstb_\intr(\cdot) \in \dfset_\intr, \state_{i, \intr}(\cdot) \text{ satisfies \eqref{eq:reldyn}},\\
& \exists s \in [t, \brd], \state_{i, \intr}(s) \in \targetset^{\text{B}}_{i}, \state_{i, \intr}(t) = y\},
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\targetset^{\text{B}}_{i} &= \{\state_{i, \intr}: \|\pos_{i, \intr}\|_2 \le \rc\} \\
H^{\text{B}}_{i}(\state_{i, \intr}, \costate) &= \min_{\ctrl_i \in \cset_i, \ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{i, \intr}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}

The interpretation of set $\brs^{\text{B}}_{i}(0, \brd)$ is that if $\state_{i, \intr}$ is outside the boundary of this set, then $\veh_{\intr}$ and $\veh_{i}$ cannot enter the danger zone $\dz_{i\intr}$ for a duration of $\brd$, irrespective of control applied by them. When $\state_{\intr}^0 \in \sep_j(\tsa)$, we can get the same property in absolute co-ordinates by augmenting this set on the separation region of the $\veh_j$
\begin{equation} \label{eqn:buffRegion}
\buff_{ij}(t) = \sep_j(t) + \brs^{\text{B}}_{i}(0, \brd),
\end{equation} 
and ensuring that $\veh_i$ is outside the boundary of $\buff_{ij}(t)$.

Finally, during the path planning of $\veh_i$, we also need to ensure that $\veh_i$ is far enough from the boundary of $\buff_{ij}(t)$ such that $\veh_{\intr}$ and $\veh_{i}$ cannot enter the danger zone $\dz_{i\intr}$ for the remaining duration of $\trd := \iat - \brd$. Thus, during the path planning of $\veh_i$, we need to ensure that $\veh_i$ is outside the augmented buffer region:
\begin{equation} \label{eqn:augbuffRegion1}
\tilde{\buff}_{ij}(t) = \buff_{ij}(t) + \brs^{\text{S}}_{i}(0, \trd),
\end{equation}
where $\brs^{\text{S}}_{i}(0, \trd)$ can be computed as described in Section \ref{sec:sepRegion}. Region $\tilde{\buff}_{ij}(t)$ is also illustrated in Figure \ref{fig:buffRegion}.

\begin{figure}[H]
  \centering
  \includegraphics[width=0.4\textwidth]{"figs/buffRegion"}
  \caption{Illustration of region $\tilde{\buff}_{ij}(t)$ (best visualized in color). The Blue region denotes the base obstacle $\boset_j(t)$ induced by $\veh_j$ at time $t$. The base obstacle is augmented by the set $\brs^{\text{S}}_{j}(0, \iat)$, denoted as the Yellow region. The region within the dotted Black boundary is thus the separation region $\sep_j(t)$. As long as the intruder is outside the dotted Black boundary, $\veh_j$ can apply any control and still guaranteed to not enter the danger zone $\dz_{j\intr}$. The separation region is augmented by $\brs^{\text{B}}_{i}(0, \brd)$, giving the buffer region $\buff_{ij}(t)$ (the region within the solid Black boundary). Finally, the buffer region is augmented by $\brs^{\text{S}}_{i}(0, \trd)$ to get $\tilde{\buff}_{ij}(t)$ (the region within the dashed Black boundary). If we make sure that $\veh_i$ is outside the dashed Black boundary, any intruder appearing at the boundary of the separation region of $\veh_j$ (dotted Black boundary) must ``travel" through the Grey region before it can reach the boundary of the separation region of $\veh_i$ (solid Black boundary). Since the Grey region is computed for a duration of $\brd$, there should atleast a gap of $\brd$ between two time instants where $\veh_{\intr}$  affects $\veh_i$ and $\veh_j$.}
  \label{fig:buffRegion}
\end{figure}

\subsubsection{Case2- $\state_{\intr}^0 \in \sep_i(\tsa)$} \label{sec:buffCase2}
This case can be treated in a similar fashion as Section \ref{sec:buffCase1}. We can now look at the same problem from $\veh_i$'s perspective and compute the augmented buffer region $\tilde{\buff}_{ji}(t)$ as:
\begin{equation} \label{eqn:augbuffRegion2}
\tilde{\buff}_{ji}(t) = \boset_j(t) + \brs^{\text{S}}_{j}(0, \trd) + \brs^{\text{B}}_{j}(0, \brd) + \brs^{\text{S}}_{i}(0, \iat).
\end{equation}
During the path planning of $\veh_i$, we also need to ensure that $\veh_i$ is outside $\tilde{\buff}_{ji}(t)$. 

==> intruder_archived_v0/intro.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\section{Response to Intruders \label{sec:intruder}}
\MCnote{Need diagrams illustrating all the different times (BRD, RD, etc.)}

\MCnote{Need to mention augmentation of static obstacles.}

In Section \ref{sec:rtt}, we presented RTT algorithm that can take into account disturbances in vehicles' dynamics. However, if a vehicle not in the set of SPP vehicles enters the system, or even worse, if this vehicle is an adversarial intruder, the original plan can lead to vehicles entering into each other's danger zones. If vehicles do not plan with an additional safety margin that takes a potential intruder into account, a vehicle trying to avoid the intruder may effectively become an intruder itself, leading to a domino effect. %In this section, we propose a method to allow vehicles to avoid an intruder while maintaining the SPP structure.

In general, the effect of an intruder on the vehicles in structured flight can be entirely unpredictable, since the intruder in principle could be adversarial in nature, and the number of intruders could be arbitrary. Therefore, we make the following two assumptions: %for our analysis to produce reasonable results, two assumptions about the intruders must be made.

\begin{assumption}
\label{as:avoidOnce}
At most one intruder (denoted as $\veh_I$ here on) affects the SPP vehicles at any given time. The intruder exits the altitude level affecting the SPP vehicles after a duration of $\iat$. 
\end{assumption}

Let the time at which intruder appears in the system be $\tsa$ and the time at which it disappears be $\tea$. Assumption \ref{as:avoidOnce} implies that $\tea \leq \tsa + \iat$. Thus, any vehicle $\veh_i$ would need to avoid the intruder $\veh_{\intr}$ for a maximum duration of $\iat$. %This assumption can be valid in situations where intruders are rare, and that some fail-safe or enforcement mechanism exists to force the intruder out of the altitude level affecting the SPP vehicles. 
Note that we do not pose any restriction on $\tsa$; however, we assume that once the intruder appears, it stays for a maximum duration of $\iat$.
%in addition, after avoiding the intruder, Qi can safely assume that it would not need to avoid another intruder

\begin{assumption}
\label{as:dynKnown}
The dynamics of the intruder are known and given by $\dot\state_\intr = f_\intr(\state_\intr, \ctrl_\intr, \dstb_\intr)$.
\end{assumption}

Assumption \ref{as:dynKnown} is required for HJ reachability analysis. In situations where the dynamics of the intruder are not known exactly, a conservative model of the intruder may be used instead. We also denote the initial state of the intruder as $\state_{\intr}^0.$ Note that $\state_{\intr}^0$ is unknown.

Our goal is to design a control policy that ensures separation with the intruder and other SPP vehicles, and ensures a successful transit to the destination. However, depending on the initial state of the intruder and its control policy, a vehicle may arrive at different states after avoiding the intruder. Therefore, a control policy that ensures a successful transit to the destination needs to account for all such possible states, which is a path planning problem with multiple initial states and a single destination, and is hard to solve in general. Thus, we divide the intruder avoidance problem into two sub-problems: (i) we first design a control policy that ensures a successful transit to the destination if no intruder appears and that successfully avoid the intruder, if it does. (ii) after the intruder disappears at $\tea$, we replan the trajectories of the affected vehicles. Following the same theme and assumptions, authors in \cite{chen2016robust} present an algorithm to avoid an intruder in SPP formulation; however, once the intruder disappears, the algorithm might need to replan the trajectories for all SPP vehicles. Since the replanning is done in real-time, it should be fast and scalable with the number of SPP vehicles, rendering the method in \cite{chen2016robust} unsuitable for practical implementation.  

In this work, we propose a novel intruder avoidance algorithm, which will need to replan trajectories only for a fixed number of vehicles, irrespective of the total number of SPP vehicles. Moreover, this number is a design parameter, which can be chosen based on the resources available during the run time. Intuitively, one can think about dividing the flight space of vehicles such that at any given time, any two vehicles are far enough from each other so that an intruder can only affect atmost $\nva$ vehicles in a duration of $\iat$ despite its best efforts. In this method, we build upon this intuition and show that such a division of space is indeed possible. The advantage of such an approach is that after the intruder disappears, we only have to replan the trajectory of \textit{atmost $\nva$} vehicles, which can be efficiently done in real-time if $\nva$ is low enough, thus making this approach particularly suitable for practical systems. %Thus the proposed method guarantees that \textit{atmost $k$} vehicles are affected by the presence of intruder, regardless of the number of SPP vehicles, and hence the replanning can be efficiently done in real-time. 

\SBnote{Fix the organization of sections once you finish writing the sections.}
In Sections \ref{sec:intruder_avoid}, we discuss the intruder avoidance control and explain the sensing range required to avoid the intruder. In Sections \ref{sec:sepRegion} and \ref{sec:buffRegion}, we compute a space division of state-space such that atmost $\nva$ vehicles need to apply the avoidance maneuver computed in Section \ref{sec:intruder_avoid}, regardless of the initial state of the intruder. However, we still need to ensure that vehicles do not collide with each other while avoiding the intruder. The induced obstacles that reflect this possibility are computed in Section \ref{sec:intruderObs}. Trajectopry planning and replanning are discussed in Sections \ref{sec:plan} and \ref{sec:replan} respectively.

==> intruder_archived_v0/obstacles.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Obstacle Computation} \label{sec:intruderObs}
In sections \ref{sec:sepRegion} and \ref{sec:buffRegion}, we computed a separation between any two vehicles, such that the intruder can affect atmost $\nva$ vehicles during a duration of $\iat$. However, we need to make sure that while applying avoidance control a vehicle does not enter the danger zone of other vehicle or collide with the static obstacles. In this section, we compute the obstacles that reflect this possibility. In particular, we want to find the set of states that a lower priority vehicle $\veh_i$ needs to avoid to avoid entering in the danger zone of a higher priority vehicle $\veh_j$, $j < i$. To find such states, we consider the following five mutually exclusive and exhaustive cases:
\begin{enumerate}
\item Intruder does not affect $\veh_j$ or $\veh_i$ during their flight.
\item Intruder affects $\veh_j$, but not $\veh_i$.
\item Intruder affects $\veh_i$, but not $\veh_j$.
\item Intruder first affects $\veh_j$ and then $\veh_i$.
\item Intruder first affects $\veh_i$ and then $\veh_j$.
\end{enumerate}
For each case, we compute the set of states that $\veh_i$ needs to avoid to avoid entering in $\dz_{ji}$. Let $^k\ioset_i^j(\cdot)$ denotes the set of obstacles corresponding to the case $k$ above. 

\subsubsection{Case1} \label{sec:intruderObs_case1}
When the intruder does not affect any of the two vehicles, $\veh_i$ simply needs to avoid the set of base obstacles $\boset_j(t)$. Therfore, 
\begin{equation} \label{eq:intruderObs_case1}
\begin{aligned}
^1\ioset_i^j(t) & = \{\state_i: \exists y \in \pfrs_j(t), \|\pos_i - y\|_2 \le \rc \}\\
\pfrs_j(t) & = \{p_j: \exists \npos_j, (p_j, \npos_j) \in \boset_j(t) \}
\end{aligned}
\end{equation}


\subsubsection{Case2} \label{sec:intruderObs_case2}
To compute the obstacles that $\veh_i$ needs to avoid at time $t$ for the remaining four cases, we start with the following observation:
\begin{observation} \label{obs0_case2}
It is sufficient to consider the scenarios where $\tsa \in [t-\iat, t]$. This is because if $\tsa < t - \iat$, then $\veh_i$ and/or $\veh_j$ will already be in the replanning phase at time $t$ (see assumption \ref{as:avoidOnce}) and hence the two vehicles cannot be in conflict at time $t$. On the other hand, if $\tsa > t$, then we need not account for the intruder as it has not appeared in the system yet. %\SBnote{Actually, we compute obstacles at time $t'$ in a way such that their effect doesn't propagate to $t < t'$, but not sure if we need to mention this.}
\end{observation}

The induced obstacles for Case2 at time $t$ are given by the states that $\veh_j$ can reach while avoiding the intruder, starting from some state in $\boset_j(\tsa), \tsa \in [t-\iat, t]$. These states can be obtained by computing a FRS from the base obstacles.
\begin{equation} \label{eq:ObsFRS_case2}
\begin{aligned}
\frs_{j}^{\mathcal{O}}(\tsa, t) = & \{y: \exists \ctrl_j(\cdot) \in \cfset_j, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(\tsa) \in \boset_j(\tsa), \\
& \state_j(t) = y\}.
\end{aligned}
\end{equation}
$\frs_{j}^{\mathcal{O}}(\tsa, t)$ represents the set of all possible states that $\veh_j$ can reach after a duration of $(t-\tsa)$ starting from inside $\boset_j(\tsa)$. This FRS can be obtained by solving the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:
\begin{equation}
\ham_{j}^{\mathcal{O}}(\state_j, \costate) = \max_{\ctrl_j \in \cset_j} \max_{\dstb_j \in \dset_j} \costate \cdot f_j (\state_j, \ctrl_j, \dstb_j).
\end{equation} 
Since $\tsa \in [t-\iat, t]$, the induced obstacles in this case can be obtained as:
\begin{equation} \label{eq:intruderObs_case2} 
\begin{aligned}
^2\ioset_i^j(t) & = \{\state_i: \exists y \in \pfrs_j(t), \|\pos_i - y\|_2 \le \rc \}\\
\pfrs_j(t) & = \{p_j: \exists \npos_j, (p_j, \npos_j) \in \bigcup_{\tsa \in [t-\iat, t]} \frs_{j}^{\mathcal{O}}(\tsa, t) \}
\end{aligned}
\end{equation}

\begin{observation} \label{obs1_case2}
Since the base obstacles represent possible states that a vehicle can be in in the absence of the intruder, the base obstacle at any time $\tau_2$ should be contained within the FRS of the base obstacle at time $\tau_1 < \tau_2$, computed forward for a duration of $(\tau_2-\tau_1).$ That is, $\boset_j(\tau_2) \subseteq \frs_{j}^{\text{BO}}(\tau_1, \tau_2)$, where $\frs_{j}^{\text{BO}}(\tau_1, \tau_2)$ denotes the FRS of $\boset_j(\tau_1)$ computed forward for a duration of $(\tau_2-\tau_1)$. The same argument can be applied for the FRS computed from $\boset_j(\tau_2)$ and $\boset_j(\tau_1)$. That is, $\frs_{j}^{\text{BO}}(\tau_2, \tau_3) \subseteq \frs_{j}^{\text{BO}}(\tau_1, \tau_3)$, where $\tau_1 < \tau_2 < \tau_3$.
%Note that by the definition of base obstacles, $\boset_j(t+\tau_2) \subset \frs_{j}^{\text{BO}}(0, \tau_2-\tau_1) ~\forall t, \tau_2 > \tau_1$, where $\frs_{j}^{\text{BO}}(0, \tau_2-\tau_1)$ denotes the FRS of $\boset_j(t+\tau_1)$ computed for a duration of $\tau_2-\tau_1$. Therefore, we have that $\frs_{j}^{\mathcal{O}}(0, \tau) \subset \frs_{j}^{\mathcal{O}}(0, \iat) ~\forall \tau \in [0, \iat)$. 
\end{observation}

Using observation \ref{obs1_case2}, $\pfrs_j(t)$ in \eqref{eq:intruderObs_case2} can be equivalently written as:
\begin{equation} \label{eq:intruderObs_case2_inter}
\pfrs_j(t) = \{p_j: \exists \npos_j, (p_j, \npos_j) \in \frs_{j}^{\mathcal{O}}(t-\iat, t) \}.
\end{equation}

\subsubsection{Case3} \label{sec:intruderObs_case3}
In this case, we need to ensure that $\veh_i$ doesn't collide with the obstacle set $\boset_j(\cdot)$ or any static obstacles even when it is avoiding the intruder. In particular, we can compute a region around the obstacles such that for all disturbances, $\veh_i$ can avoid colliding with them for $\iat$ seconds regardless of its control, if $\veh_i$ starts outside this region. 

Suppose that the intruder appears in the system at time $\tsa := t - \iat + \tau, \tau \in [0, \iat]$. In this case, $veh_i$ might be applying avoidance control during the interval $[t - \iat + \tau, t + \tau]$. Thus, we need to ensure that $\veh_i$ does not collide with the obstacle $\boset_j(t + t')$ at time $t + t'$, $t' \in [t, t + \tau]$, regardless of its control $\ctrl_i(s)$ and disturbance $\dstb_i(s)$ for the time interval $s \in [\tsa, t']$. It is, therefore, sufficient to avoid the $t'$-horizon BRS of $\boset_j(t + t')$ at time $t$. This argument applies for all $t' \in [t, t + \tau]$. Thus, for a given $\tau$, we need to avoid the BRS $\brs^{\mathcal{G}}_{i}(t, t+\tau)$:
\begin{equation}  \label{eq:ObsBRS_case3}
\begin{aligned}
\brs^{\mathcal{G}}_{i}(t, t+\tau) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \exists s \in [t, t+\tau], \state_i(s) \in \tilde{\boset}_j(s) \cup \soset_i \}, \\
\tilde{\boset}_j(s) = & \{\state_j: \exists (y, h) \in \boset_j(s), \|\pos_j - y\|_2 \le \rc \}.
\end{aligned}
\end{equation}
The Hamiltonian $\ham^{\mathcal{G}}_{i}$ to compute $\brs^{\mathcal{G}}_{i}(\cdot)$ is given by:
\begin{equation} \label{eqn:BRS_obsham}
\ham^{\mathcal{G}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i).
\end{equation}

Finally, the induced obstacles in this case can be computed by taking into account all possible $\tau \in [0, \iat]$.
\begin{equation} \label{eq:intruderObs_case3}
\begin{aligned}
^3\ioset_i^j(t) = & \bigcup_{\tau \in [0, \iat]} \brs^{\mathcal{G}}_{i}(t, t+\tau)\\
= & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \exists s \in [t, t+\iat], \state_i(s) \in \tilde{\boset}_j(s) \cup \soset_i \}.
\end{aligned}
\end{equation}

The obstacle computation (sans static obstacles) is illustrated in Figure \ref{fig:obsCase3}.
\begin{figure}[H]
  \centering
  \includegraphics[width=0.5\textwidth]{"figs/obsCase3"}
  \caption{The Red and Green sets denote the base obstacles $\boset_j(\cdot)$ induced by $\veh_j$. They are augmented by the capture radius $\rc$ to get $\tilde{\boset}_j(\cdot)$ (denoted by dotted and solid lines). When $\tsa = t - \iat + \tau_1$, $\veh_i$ might be applying avoidance control during the interval $[t - \iat + \tau_1, t + \tau_1]$; therefore, it must avoid the Red obstacles during the time interval $[t, t + \tau_1]$. Equivalently, $\veh_i$ needs to avoid $\brs^{\mathcal{G}}_{i}(t, t+\tau_1)$ at time $t$. Similarly, if $\tsa = t - \iat + \tau_2$, $\veh_i$ needs to avoid Red obstacles during $[t, t + \tau_1]$ and Green obstacles during $[t + \tau_1, t + \tau_2]$. This is precisely what set $\brs^{\mathcal{G}}_{i}(t, t+\tau_2)$ captures.}
  \label{fig:obsCase3}
\end{figure}

\subsubsection{Case4} \label{sec:intruderObs_case4}
In this case, $\state_{\intr}^0 \in \partial\sep_j(\tsa)$ (by virtue of Observation \ref{obs1_buffReg}). Since $\veh_{\intr}$ affects both $\veh_i$ and $\veh_j$ in this case, we must also have $\state_{\intr}(t') \in \partial\sep_i(t')$ for some $t' \in [\tsa, \tea]$.

After forcing $\veh_j$ to apply avoidance control for some duration, 

 $t_1 \in \mathbb{R}$, it reaches at the boundary of set $\sep_i(\tsa + t_1 + t_2)$ at time $(\tsa + t_1 + t_2) \in \mathbb{R}$. Once $\veh_j$ starts applying avoidance control at time $\tsa$, it might deviate from its planned trajectory. From the perspective of $\veh_i$, $\veh_j$ can apply any control for the next $\iat$ duration. Furthermore, $\veh_i$ itself might need to apply avoidnace maneuver starting at time $(\tsa + t_1 + t_2)$ and hence to compute obstacles in this case, we need to make sure that $\veh_i$ does not collide with $\veh_j$ when $\veh_j$ has deviated from its original trajectory \textit{and} $\veh_i$ is avoiding the intruder.   

To compute the induced obstacles in this case, we first make the following observations:
\begin{observation} \label{obs1_case4}
To compute the induced obstacle at time $t$ for this case, it is sufficient to consider the scenario where $t_1 + t_2 \leq t - \tsa \leq \iat$. If $t - \tsa < t_1 + t_2$, then at time $t$, $\veh_i$ does not need to avoid the intruder as it is not on the boundary of $\sep_i(t)$. Thus, $\veh_i$ only needs to make sure that it does not enter the danger zone of $\veh_j$, which has already been ensured in Case2. 
\end{observation}
\begin{observation} \label{obs2_case4}
By the design of buffer region in Section \ref{sec:buffRegion}, we have that $t_2 \geq \brd$. Combining this fact with observation \ref{obs1_case4} implies that $t- \tsa \geq \brd$.
\end{observation}

While avoiding the intruder, $\veh_j$ can reach any state starting from some state in $\boset_j(\tsa), \tsa \in [t-\iat, t]$. These states can be obtained by computing a FRS from the base obstacles as in \eqref{eq:ObsFRS_case2}. To avoid these unsafe states, $\veh_i$ needs to avoid all the states at time $t$ that can maneuver it to an unsafe state under some control. The set of states that $\veh_i$ needs to avoid can thus be given by the BRS of the unsafe states:
\begin{equation}  \label{eq:ObsBRS_case4}
\begin{aligned}
\brs^{\text{C4}}_{i}(t, \tsa + \iat) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \exists s \in [t, \tsa + \iat], \state_i(s) \in \tilde{\frs}_j^{\text{C4}}(\tsa, s)\},
\end{aligned}
\end{equation}
where
\begin{equation} \label{eq:ObsFRS_case4}
\begin{aligned}
\tilde{\frs}_{j}^{\text{C4}}(t', s) & = \{\state_j: \exists (y, h) \in \frs_j^{\text{C4}}(t', s), \|\pos_j - y\|_2 \le \rc \},\\
\frs_j^{\text{C4}}(t', s) & = \{y: \exists \ctrl_j(\cdot) \in \cfset_j, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(t') \in \boset_j(t'), \\
& \state_j(s) = y\}.
\end{aligned}
\end{equation} 
The Hamiltonian $\ham^{\text{C4}}_{i}$ to compute $\brs^{\text{C4}}_{i}(\cdot)$ is given by:
\begin{equation} \label{eqn:BRS_obsham}
\ham^{\text{C4}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i).
\end{equation}
Finally, the induced obstacle in this case can be obtained as:
\begin{equation} \label{eq:intruderObs_case4_alt1} 
^4\ioset_i^j(t) = \bigcup_{\tau \in [0, \iat - \brd]} \brs^{\text{C4}}_{i}(t, t + \tau),
\end{equation}
where range of $\tau$ is obtained via observation \ref{obs2_case4}.

Finally, by the definition of base obstacles, we have that $\frs_j^{\text{C4}}(t', s) \subseteq \frs_j^{\text{C4}}(t'', s), ~\forall t' > t''$. The union in \eqref{eq:intruderObs_case4_alt1} can thus be obtained by computing a single BRS:
\begin{equation} \label{eq:intruderObs_case4} 
\begin{aligned}
^4\ioset_i^j(t) & = \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \exists s \in [t, t + \iat - \brd], \state_i(s) \in \tilde{\frs}_j^{\text{C4}}(s-\iat, s)\}.
\end{aligned}
\end{equation}

\subsubsection{Case5} \label{sec:intruderObs_case5}
In this case, intruder $\veh_{\intr}$ appears at the boundary of set $\sep_i(\tsa)$ and after forcing $\veh_i$ to apply avoidance control for some duration $t_1 \in \mathbb{R}$, it reaches at the boundary of set $\sep_j(\tsa + t_1 + t_2)$ at time $(\tsa + t_1 + t_2) \in \mathbb{R}$. Similar to Case4, once $\veh_i$ starts applying avoidance control at time $\tsa$, it might deviate from its planned trajectory. $\veh_j$ itself might need to apply avoidnace maneuver starting at time $(\tsa + t_1 + t_2)$ and hence to compute obstacles in this case, we need to make sure that $\veh_i$ does not collide with $\veh_j$ when $\veh_j$ is avoiding the intruder \textit{and} $\veh_i$ has deviated from its original trajectory. It is, therefore, sufficent that $\veh_i$ avoids the following BRS:
\begin{equation}  \label{eq:ObsBRS_case5}
\begin{aligned}
\brs^{\text{C5}}_{i}(t, \tsa + \iat) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \exists s \in [t_M, \tsa + \iat], \state_i(s) \in \tilde{\frs}_j^{\text{C5}}(\tsa+t_1+t_2, s)\},
\end{aligned}
\end{equation}
where
\begin{equation} \label{eq:ObsAltSet_case5}
\begin{aligned}
t_M & = max(\tsa+t_1+t_2, t),\\
\tilde{\frs}_{j}^{\text{C5}}(t', s) & = \{\state_j: \exists (y, h) \in \frs_j^{\text{C5}}(t', s), \|\pos_j - y\|_2 \le \rc \},\\
\frs_j^{\text{C5}}(t', s) & = \{y: \exists \ctrl_j(\cdot) \in \cfset_j, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(t') \in \boset_j(t'), \\
& \state_j(s) = y\}.
\end{aligned}
\end{equation} 
The Hamiltonian $\ham^{\text{C5}}_{i}$ to compute $\brs^{\text{C5}}_{i}(\cdot)$ is given by:
\begin{equation} \label{eqn:BRS_obsham}
\ham^{\text{C5}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i).
\end{equation}   

The above set can be interpreted as follows: $\frs_j^{\text{C5}}$ represents the states that $\veh_j$ might be in while avoiding the intruder. Thus to avoid these states, it is sufficient to avoid the BRS of $\frs_j^{\text{C5}}$ (after taking into account the danger zone $\dz_{ij}$) at time $t$, which is given by $\brs^{\text{C5}}_{i}$. Therefore, the induced obstacle in this case can be obtained by taking into account all possible $\tsa, t_1$ and $t_2$:
\begin{equation} \label{eq:intruderObs_case5_alt1} 
^5\ioset_i^j(t) = \bigcup_{\tsa \in [t-\iat, t], t_2 \geq \brd, t_1 + t_2 \in (0, \iat)} \brs^{\text{C5}}_{i}(t, \tsa + \iat),
\end{equation}
where range of $t_2$ is obtained via observation \ref{obs2_case4} and $t_1 + t_2 \leq \iat$ is implied due to assumption \ref{as:avoidOnce}.

Next we make the following observations:
\begin{observation} \label{obs1_case5}
By definition of the base obstacles, $\boset_j(t') \subseteq \frs_j^{\text{BO}}(t'', t')$, where $t'' < t'$ and $\frs_j^{\text{BO}}$ represents the FRS of the base obstacle $\boset_j(t'')$ computed for a duration of $t' - t''$. Therefore, for a given $\tsa$ and $t_2$, we have $\tilde{\frs}_j^{\text{C5}}(\tsa+t_1+t_2, s) \subseteq \tilde{\frs}_j^{\text{C5}}(\tsa+t_2, s) ~\forall t_1 >0$. Therefore, the biggest obstacles are induced for $\veh_i$ when $t_1 = 0$ and hence for the obstacle computation purposes we can assume that $t_1 = 0$. Similar argument can be applied for $t_2$. Therefore, we can assume that $t_2 = \brd$. 
\end{observation}

\begin{observation} \label{obs2_case5}
If $\tsa < t- 2\brd$, then $\tsa + t_1 + t_2 < t - \brd$ (see Observation \ref{obs1_case5}). That is $\veh_j$ applies the avoidance maneuver atleast for a duration of $\brd$ before time $t$. Thus, the intruder have enough time before it must disappear to travel through the buffer region and affect $veh_i$ again. But this scenario is already covered in Case4. So for Case5, we can safely assume that $\tsa \in [t-2*\brd, t]$. 
\end{observation}
Using the above two observations, the induced obstacle and $\brs^{\text{C5}}_{i}$ can be re-written as:
\begin{equation} \label{eq:intruderObs_case5} 
\begin{aligned}
^5\ioset_i^j(t) = & \bigcup_{\tau \in [t+\iat -2\brd, t+\iat]} \brs^{\text{C5}}_{i}(t, \tau),\\
\brs^{\text{C5}}_{i}(t, \tau) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(t) = y, \\
& \state_i(\tau) \in \tilde{\frs}_j^{\text{C5}}(\tau-\iat+\brd, \tau)\}.
\end{aligned}
\end{equation}

==> intruder_archived_v0/plan.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Optimal Avoidance Controller} \label{sec:intruder_avoid}
Given the separation and buffer regions and induced obstacles, the overall obstacle for $\veh_i$ is given by:
\begin{equation}
\label{eq:obsseti_intr}
\obsset_i(t)  = \soset_i \cup \bigcup_{j=1}^{i-1} \left( \tilde{\buff}_{ij}(t) \cup \tilde{\buff}_{ji}(t) \cup_{k=1}^{5} {^k\ioset_i^j}(t) \right)
\end{equation}

Given $\obsset_i(t)$, we compute a BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ for path planning that contains the initial state of $\veh_i$ while avoiding these obstacles:
\begin{equation} \label{eqn:intrBRS1}
\begin{aligned}
\brs^{\text{AO}}_{i}(t, \sta_i) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \forall \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \forall s \in [t, \sta_i], \state_i(s) \notin \obsset_i(s), \\
& \exists s \in [t, \sta_i], \state_i(s) \in \targetset_i, \state_i(t) = y \}.
\end{aligned}
\end{equation}
The Hamiltonian $\ham^{\text{AO}}_{i}$ to compute BRS in \eqref{eqn:intrBRS1} is given by:
\begin{equation} \label{eqn:BRSham}
\ham^{\text{AO}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

Note that $\brs^{\text{AO}}_{i}(\cdot)$ ensures goal satisfaction for $\veh_i$ in the absence of intruder. The goal satisfaction controller is given by:
\begin{equation}
{\ctrl^{\text{AO}}_{i}}(t, \state_i) = \arg \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}
Moreover, if $\veh_i$ starts within $\brs^{\text{AO}}_{i}$, it is guaranteed to avoid collision with other vehicles for a duration of $\iat$, starting at any $\tsa < \sta_i$, irrespective of the control and disturbance applied by vehicles (including $\veh_i$ itself) during this time period. 

\begin{remark}
Note that if we use the robust trajectory tracking method to compute the base obstacles, we would need to augment the obstacles in \eqref{eq:obsseti_intr} by the error bound of $\veh_i$, $\disckernel_i$, as discussed in section \ref{sec:rtt}.
\end{remark}

To compute the optimal avoidance control for $\veh_i$ in presence of $\veh_{\intr}$, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_i$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. Given the relative dynamics in \eqref{eq:reldyn}, this set of states is given by the BRS $\brs^{\text{S}}_{i}(\tau, \iat),~ \tau \in [0, \iat]$, given by \eqref{eqn:sepBRS}.

Once the value function $\valfunc^{\text{S}}_{i}(\cdot)$ is computed, the optimal avoidance control ${\ctrl^{\text{S}}_{i}}$ can be obtained as:
\begin{equation} \label{eqn:optAvoidCtrl}
{\ctrl^{\text{S}}_{i}} = \arg \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{equation}

Under normal circumstances when the intruder $\veh_{\intr}$ is far away, we have $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) > 0$; as $\veh_{\intr}$ gets closer to $\veh_i$, $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t))$ decreases. If $\veh_i$ applies the control ${\ctrl^{\text{S}}_{i}}$ when $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) = 0$, then collision avoidance between $\veh_i$ and $\veh_{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

In addition, computation of $\obsset_i(\cdot)$ ensures that $\veh_i$ does not collide with any other SPP vehicle during the avoidance maneuver. %Therefore, applying $\ctrl_I^A$ for a duration of $\iat$ is still guaranteed to keep $\veh_i$ safe from all obstacles, and hence safe from collision with respect to all other vehicles $\veh_j, j \neq i$.
The overall control policy for avoiding the intruder and collision with other vehicles is thus given by:
\begin{equation*}
{\ctrl^{\text{A}}_{i}}(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{AO}}_{i}}(t) & t \leq \tsa\\
{\ctrl^{\text{S}}_{i}}(t) & \tsa\leq t \leq \tea
\end{array}
\right.
\end{equation*}

\SBnote{Somewhere mention the conditions under which our method is guaranteed to avoid the intruder.} 

==> intruder_archived_v0/replan.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Replanning after intruder avoidance} \label{sec:replan}
Intruder can force some SPP vehicles to deviate from their planned trajectory; therefore, we have to replan the trajectory of these vehicles once $\veh_{intr}$ disappears. The set of all vehicles $\veh_i$ for whom we need to replan the trajectories, $\rvs$, can be obtained by checking if a vehicle $\veh_i$ applied any avoidnace control during $[\tsa, \tea]$, e.g.,
\begin{equation} \label{eq:RVS}
\rvs = \{\veh_i, i \in \{1, \ldots, \N \}: \valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) \leq 0, t \in [\tsa, \tea] \}. 
\end{equation}  

Note that due to the presence of separation and buffer regions, atmost $\nva$ vehicles can be affected by $\veh_{intr}$, e.g. $|\rvs| \leq \nva$. Goal satisfaction controllers which ensure that these vehicles reach their destinations can be obtained by solving a new SPP problem, where the starting states of the vehicles are now given by the states they end up in, denoted $\tilde{\state}_i^0$, after avoiding the intruder. Let the optimal control policy corresponding to this liveness controller be denoted ${\ctrl^{\text{L}}_{i}}(t, \state_i)$. The overall control policy that ensures intruder avoidance, collision avoidance with other vehicles, and successful transition to the destination for vehicles in $\rvs$ is given by:

\begin{equation*}
\ctrl_i^*(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{A}}_{i}}(t, \state_i) & t \leq \tea\\
{\ctrl^{\text{L}}_{i}}(t, \state_i) & t > \tea
\end{array}
\right.
\end{equation*}

Note that in order to re-plan using a SPP method, we need to determine feasible $\sta_i$ for all vehicles. This can be done by computing an FRS:
\begin{equation} \label{eq:re-planFRS}
\begin{aligned} 
\frs_i^{\text{RP}}(\tea, t) = & \{y \in \R^{n_i}: \exists \ctrl_i(\cdot) \in \cfset_i, \forall \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(\tea) = \tilde{\state}_i^0, \\
& \state_i(t) = y, \forall s \in [\tea, t], \state_i(s) \notin \obsset_i^{\text{RP}}(s) \},
\end{aligned}
\end{equation}
\noindent where $\tilde{\state}_i^0$ represents the state of $\veh_i$ at $t = \tea$; $\obsset_i^{\text{RP}}(\cdot)$ takes into account the fact that $\veh_i$ needs to avoid higher-priority vehicles $\veh_j, j<i$ and is defined in an way analogous to \eqref{eq:obsseti}.
%\begin{equation} 
%\obsset_j^{\text{RP}}(t) = \bigcup_{k<j} \frs_k^{\text{RP}}(\tea, t), ~~~t > \tea.
%\end{equation}

The FRS in \eqref{eq:re-planFRS} can be obtained by solving %the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:

\begin{equation}
\begin{aligned}
\max \Big\{&D_t \valfuncfwd_i^{\text{RP}}(t, \state_i) + \ham_i^{\text{RP}}(t, \state_i, \nabla \valfuncfwd_i^{\text{RP}}(t, \state_i)), \\
&\qquad - \obsfunc_i^{\text{RP}}(t, \state_i) - \valfuncfwd_i^{\text{RP}}(t, \state_i) \Big\} = 0\\
&\valfuncfwd_i^{\text{RP}}(\tsa, \state_i) = \max\{\fc_i^{\text{RP}}(\state_i), -\obsfunc_i^{\text{RP}}(\tsa, \state_i)\} \\
&\ham_i^{\text{RP}}(\state_i, \costate) = \max_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{aligned}
\end{equation} 

\noindent where $\valfuncfwd_i^{\text{RP}}, \obsfunc_i^{\text{RP}}, \fc_i^{\text{RP}}$ represent the FRS, obstacles during re-planning, and the initial state of $\veh_i$, respectively. The new $\sta$ of $\veh_i$ is now given by the earliest time at which $\frs_i^{\text{RP}}(\tea, t)$ intersects the target set $\targetset_i$, $\sta_i := \arg \inf_t \{ \frs_i^{\text{RP}}(\tea, t) \cap \targetset_i \neq \emptyset \}$. Intuitively, this means that there exists a control policy which will steer the vehicle $\veh_i$ to its destination by that time, despite the worst case disturbance it might experience.

\begin{remark}
Note that even though we have presented the analysis for one intruder, the proposed method can handle multiple intruders as long as only one intruder is present \textit{at any given time}. 
\end{remark}

We conclude this section with the overall SPP algorithm that takes into account an intruder that may appear for a duration of $\iat$: 
\begin{alg}
\label{alg:intruder}
\textbf{Intruder Avoidance algorithm (offline planning)}: Given initial conditions $\state_i^0$, vehicle dynamics \eqref{eq:dyn}, intruder dynamics in Assumption \ref{as:dynKnown}, target sets $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$, for each $i$,
\begin{enumerate}
\item determine the separation region and buffer regions given by \eqref{eqn:sepRegion}, \eqref{eqn:augbuffRegion1} and \eqref{eqn:augbuffRegion2}.
\item compute the induced obstacles for $\veh_i$ by $\veh_j$ given by \eqref{eq:intruderObs_case1}, \eqref{eq:intruderObs_case2}, \eqref{eq:intruderObs_case3}, \eqref{eq:intruderObs_case4} and \eqref{eq:intruderObs_case5}. 
\item compute the total obstacle set $\obsset_i(t)$, given in \eqref{eq:obsseti_intr}. In the case $i=1$, $\obsset_i(t) = \soset_i ~ \forall t$;
\item given $\tilde\obsset_i(t)$, compute the BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ defined in \eqref{eqn:intrBRS1};
\item the optimal control to avoid the intruder can be obtained by using \eqref{eqn:optAvoidCtrl};
\end{enumerate}

\textbf{Intruder Avoidance algorithm (online re-planning)}: For each vehicle $\veh_i \in \rvs$ which performed avoidance in response to the intruder,
\begin{enumerate}
\item compute $\frs_i^{\text{RP}}(\tea, t)$ using $\eqref{eq:re-planFRS}$. The new $\sta_i$ for $\veh_i$ is given by $\arg \inf_t \{ \frs_j^{\text{RP}}(\tea, t) \cap \targetset_j \neq \emptyset \}$;
\item given $\sta_i$, $\tilde{\state}_i^0$, vehicle dynamics \eqref{eq:dyn}, target set $\targetset_i$, and obstacles $\obsset_i^{\text{RP}}$, use any of the three SPP methods discussed in \cite{chen2016robust} for re-planning. 
\end{enumerate}
\end{alg}

==> intruder_archived_v0/sepRegion.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Separation Region} \label{sec:sepRegion}
Depending on the information known to a lower-priority vehicle $\veh_i$ about $\veh_j$'s control strategy, we can use one of the three methods described in Section 5 in \cite{chen2016robust} to compute the ``base" obstacles $\boset_j(t)$, the obstacles that would have been induced by $\veh_j$ in the presence of disturbances, but in the absence of an intruder. The base obstacles are respectively given by equations (25), (31) and (37) in \cite{chen2016robust} for centralized control, least restrictive control and robust trajectory tracking algorithms.

Given $\boset_j(t)$, we compute the set of all states of the intruder for which vehicle $\veh_j$ may have to apply an avoidnace maneuver. We refer to this set as \textit{separation region} here on, and denote it as $\sep_j(t)$. The significance of $\sep_j(t)$ is that as long as the intruder is outside $\sep_j(t)$, that is $\state_{\intr}(t) \in \left(\sep_j(t)\right)^c$, $\veh_j$ can apply any control at time $t$ and still guaranteed to not collide with the intruder. $\sep_j(t)$ can be conveniently computed using the relative dynamics between $\veh_j$ and $\veh_{\intr}$. 

We define relative dynamics of the intruder $\veh_{\intr}$ with state $\state_\intr$ with respect to $\veh_i$ with state $\state_i$:
\begin{equation}
\label{eq:reldyn}
\begin{aligned}
\state_{\intr, i} &= \state_\intr - \state_i \\
\dot \state_{\intr, i} &= f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}
Given the relative dynamics, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_{j}$ can enter danger zone $\dz_{j\intr}$ in a duration of $\iat$ despite the best efforts of $\veh_j$ to avoid $\veh_{\intr}$. Under the relative dynamics \eqref{eq:reldyn}, this set of states is given by the backwards reachable set $\brs^{\text{S}}_j(\tau, \iat)$:

\begin{equation} \label{eqn:sepBRS}
\begin{aligned}
\brs^{\text{S}}_{j}(\tau, \iat) = & \{y: \forall \ctrl_j(\cdot) \in \cfset_j, \exists \ctrl_\intr(\cdot) \in \cfset_\intr, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \exists \dstb_\intr(\cdot) \in \dfset_\intr, \state_{\intr, j}(\cdot) \text{ satisfies \eqref{eq:reldyn}},\\
& \exists s \in [\tau, \iat], \state_{\intr, j}(s) \in \targetset^{\text{S}}_{j}, \state_{\intr, j}(\tau) = y\},
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\targetset^{\text{S}}_{j} = & \{\state_{\intr, j}: \|\pos_{\intr, j}\|_2 \le \rc\} \\
H^{\text{S}}_{j}(\state_{\intr, j}, \costate) = & \max_{\ctrl_j \in \cset_j} \left( \right.\\
&\left. \min_{\ctrl_\intr \in \cset_\intr, \dstb_j \in \dset_j, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, j}, \ctrl_j, \ctrl_\intr, \dstb_j, \dstb_\intr) \right)
\end{aligned}
\end{equation}

The interpretation of set $\brs^{\text{S}}_{j}(0, \iat)$ is that as long as $\veh_{\intr}$ is outside the boundary of this set (in relative coordinates), then $\veh_{\intr}$ and $\veh_{j}$ cannot enter the danger zone $\dz_{j\intr}$, irrespective of control applied by them. But once $\veh_{\intr}$ is on the boundary of this set, then $\veh_{j}$ needs to apply the optimal avoidance control to avoid collision with $\veh_{\intr}$. We can now transform $\brs^{\text{S}}_{j}(0, \iat)$ to absolute coordinates to obtain sets $\sep_j(\cdot)$ as follows:
\begin{equation} \label{eqn:sepRegion}
\sep_j(t) = \boset_j(t) + \brs^{\text{S}}_{j}(0, \iat),
\end{equation}
where the ``$+$'' in \eqref{eqn:sepRegion} denotes the Minkowski sum.

==> intruder_archived_v1/Case1/buffRegion.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Buffer Region} \label{sec:buffRegion_case1}
$\veh_i$ is forced to apply an avoidance maneuver at time $t$ only if $\state_{\intr, i}(t) \in \partial \brs^{\text{A}}_{i}(t-\tsa, \iat)$.  


\SBnote{Start from here.}


==> intruder_archived_v1/Case1/sepRegion.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsubsection{Separation region} \label{sec:sepRegion_case1}
In this section, we find the set of all states $\state_{\intr}(t)$ for which $\veh_j$ is forced to apply an avoidnace maneuver for a given $\tsa$. We refer to this set as \textit{separation region}, and denote it as $\sep_j(\tsa, t)$. As discussed in Section \ref{sec:intruder_avoid}, $\veh_j$ needs to apply avoidnace maneuver at time $t$ only if $\state_{\intr, j}(t) \in \partial \brs^{\text{A}}_{j}(t-\tsa, \iat)$. To compute set $\sep_j(\tsa, t)$, we thus need to translate this set in relative coordinates to absolute coordinates, for which we need to know all possible states of $\veh_j$ at time $t$.

Depending on the information known to a lower-priority vehicle $\veh_i$ about $\veh_j$'s control strategy, we can use one of the three methods described in Section 5 in \cite{chen2016robust} to compute the ``base" obstacles $\boset_j(t)$, the obstacles that would have been induced by $\veh_j$ in the presence of disturbances, but in the absence of an intruder. The base obstacles are respectively given by equations (25), (31) and (37) in \cite{chen2016robust} for centralized control, least restrictive control and robust trajectory tracking algorithms.

Given $\boset_j(t)$, we compute the set of all possible states of $\veh_j$ at time $t$ given $\tsa$. Regardless of the avoidnace control applied by $\veh_j$ during $[\tsa, t]$, $\state_j(t)$ will still be contained withing the FRS $\frs^{\text{S}}_{j}(\tsa, \iat)$:  
\begin{equation} \label{eq:sepRegionFRS_case1}
\begin{aligned}
\frs_{j}^{\text{S}}(\tsa, t) = & \{y: \exists \ctrl_j(\cdot) \in \cfset_j, \exists \dstb_j(\cdot) \in \dfset_j, \\
& \state_j(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_j(\tsa) \in \boset_j(\tsa), \\
& \state_j(t) = y\}.
\end{aligned}
\end{equation}
$\frs_{j}^{\text{S}}(\tsa, t)$ represents the set of all possible states that $\veh_j$ can reach after a duration of $(t-\tsa)$ starting from inside $\boset_j(\tsa)$. This FRS can be obtained by solving the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:
\begin{equation}
\ham_{j}^{\text{S}}(\state_j, \costate) = \max_{\ctrl_j \in \cset_j} \max_{\dstb_j \in \dset_j} \costate \cdot f_j (\state_j, \ctrl_j, \dstb_j).
\end{equation} 
Thus, $\sep_j(\tsa, t)$ can be obtained as:
\begin{equation} \label{eqn:sepRegion_case1}
\sep_j(\tsa, t) = \frs_{j}^{\text{S}}(\tsa, t) + \brs^{\text{A}}_{j}(t-\tsa, \iat), ~\tsa \in [t-\iat, t],
\end{equation}
where the ``$+$'' in \eqref{eqn:sepRegion_case1} denotes the Minkowski sum.

==> intruder_archived_v1/avoid_control.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Optimal Avoidance Controller} \label{sec:intruder_avoid}
To compute the optimal avoidance control for $\veh_i$ in presence of $\veh_{\intr}$, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_i$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. 

We define relative dynamics of the intruder $\veh_{\intr}$ with state $\state_\intr$ with respect to $\veh_i$ with state $\state_i$:
\begin{equation}
\label{eq:reldyn}
\begin{aligned}
\state_{\intr, i} &= \state_\intr - \state_i \\
\dot \state_{\intr, i} &= f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr)
\end{aligned}
\end{equation}
Given the relative dynamics, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_{i}$ can enter danger zone $\dz_{i\intr}$ in a duration of $\iat$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. Under the relative dynamics \eqref{eq:reldyn}, this set of states is given by the backwards reachable set $\brs^{\text{A}}_i(\tau, \iat),~ \tau \in [0, \iat]$:

\begin{equation} \label{eqn:avoidBRS}
\begin{aligned}
\brs^{\text{A}}_{i}(\tau, \iat) = & \{y: \forall \ctrl_i(\cdot) \in \cfset_i, \exists \ctrl_\intr(\cdot) \in \cfset_\intr, \exists \dstb_i(\cdot) \in \dfset_i, \\
& \exists \dstb_\intr(\cdot) \in \dfset_\intr, \state_{\intr, i}(\cdot) \text{ satisfies \eqref{eq:reldyn}},\\
& \exists s \in [\tau, \iat], \state_{\intr, i}(s) \in \targetset^{\text{A}}_{i}, \state_{\intr, i}(\tau) = y\},
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}
\targetset^{\text{A}}_{i} = & \{\state_{\intr, i}: \|\pos_{\intr, i}\|_2 \le \rc\} \\
H^{\text{A}}_{i}(\state_{\intr, i}, \costate) = & \max_{\ctrl_i \in \cset_i} \left( \right.\\
&\left. \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{aligned}
\end{equation}

We refer to $\brs^{\text{A}}_i(\tau, \iat)$ as \textit{avoid region} hereon. Once the value function $\valfunc^{\text{A}}_{i}(\cdot)$ is computed, the optimal avoidance control ${\ctrl^{\text{A}}_{i}}$ can be obtained as:
\begin{equation} \label{eqn:optAvoidCtrl}
{\ctrl^{\text{A}}_{i}} = \arg \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{equation}

Let $\partial \brs^{\text{A}}_{i}(\cdot, \iat)$ denotes the boundary of the set $\brs^{\text{A}}_{i}(\cdot, \iat)$. The interpretation of $\brs^{\text{A}}_{i}(\tau, \iat)$ is that if $\state_{\intr, i}(t) \in \partial \brs^{\text{A}}_{i}(\tau, \iat)$, then $\veh_i$ can successfully avoid the intruder for a duration of $(\iat - \tau)$ using the optimal avoidance control in \eqref{eqn:optAvoidCtrl}. In the worst case, $\veh_i$ might need to avoid the intruder for a duration of $\iat$; thus, we must have that  
$\state_{\intr, i}(\tsa) \in \left(\brs^{\text{A}}_{i}(0, \iat)\right)^C$. Equivalently, every SPP vehicle should be able to detect the intruder at a distance of $\dsen$, where
\begin{equation} \label{eqn:sen_distance}
\dsen = \max\{ \|a\|: a \in \brs^{\text{A}}_{i}(0, \iat) \}.
\end{equation} 
Hereon, we assume that every SPP vehicle can detect the intruder at a distance of $\dsen$.

%Under normal circumstances when the intruder $\veh_{\intr}$ is far away, we have $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) > 0$; as $\veh_{\intr}$ gets closer to $\veh_i$, $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t))$ decreases. If $\veh_i$ applies the control ${\ctrl^{\text{S}}_{i}}$ when $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) = 0$, then collision avoidance between $\veh_i$ and $\veh_{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

==> intruder_archived_v1/case1.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Separation and Buffer Regions- Case1} \label{sec:case1}

\SBnote{
\begin{itemize}
\item Introduction of the section:
\begin{itemize}
\item Main summary: In the next two sections, we are computing separation between any two vehicles such that only one applies the avoidnace maneuver at a time and atmost $\nva$ vehicles need to apply avoidnace maneuver during the entire duration. 
\item To understand what this means we introduce the notation of avoid start time. Introduce the notation and give its mathematical definition in terms of relative state and avoidnace set computed in the previous section. Now explain that only one vehicle need to apply avoidance control at a time is equivalent to $t_i \neq t_j$. Only $\nva$ vehicles need to apply avoidnace control is equivalent to $t_i - t_j \geq \brd$.  
\item If we find the set of all states of $\veh_i$ such that this separation is ensured between $\veh_i$ and $\veh_m$ for all $m<i$, then during the path planning of $\veh_i$, we can then ensure that $\veh_i$ is indeed in one of these states and we will be done (as the path planning is sequential). So we next focus on finding all the states of $\veh_i$ at time $t$ such that this separation is ensured between two vehicles $\veh_j$ and $\veh_i$, $j <i$ at time $t$ for all intruding scenarios.
\end{itemize}
\item Section1: $t_j < t_i$.
\begin{itemize}
\item We next make the following observations: (1) it is sufficient to consider the scenarios where $\tsa$ is within $\iat$ distance. (2) WLOG, initial state of the intruder belongs to a boundary of vehicle $j$.
\item Section11: First find the set of all states of intruder for which $\veh_j$ is forced to apply an avoidance maneuver. Explain what that set is in relative co-ordinates for different $\tsa$. To compute the set in absolute co-ordinates we need to augment the relative states to the states of $\veh_j$. Explain, how we can compute these states of $\veh_j$ (by FRS).
\item Section12: Next we want to make sure that $\veh_i$ is far away from this set such that the intruder will need atleast a duration of $\brd$ to reach any state such that $\state_{\intr,i}$ is on the boundary of the avoid set of $\veh_i$. In relative co-ordinates, if we compute min-min set and augment it on set in Section 11, and ensure that the boundary of the avoid region is outside this augmented set then we are done. Draw a table listing the duration of each set. Mention the duration relationships. Draw a diagram showing different sets. 
\item Section13: Obstacle computation. First compute the directly induced obstacle by $\veh_j$ at time $t$ for all possible $\tsa$. Then compute the obstacle that $\veh_i$ need to avoid at any future time for different $\tsa$. Therefore, compute the BRS that it needs to avoid at $\tsa$.    
\end{itemize}
\item Section2: $t_i < t_j$.
\end{itemize}
}

In the next two sections, our goal is to ensure that any two vehicles are separated enough from each other so that %only one of the vehicles is \textit{forced} to apply the intruder avoidance maneuver at any given time. Moroever, 
atmost $\nva$ vehicles should be \textit{forced} to apply avoidnace maneuver during the duration $[\tsa, \tea]$. To capture this mathematically, for every vehicle $\veh_m$, we define 
\begin{equation*}
\avoidt_{m} := \{t: \state_{\intr,m}(t) \in \brs^{\text{A}}_{m}(t-\tsa, \iat), t \in [\tsa, \tea]\}
\end{equation*} 
$\avoidt_{m}$ is the set of all times at which $\veh_m$ is forced to apply an intruder avoidance maneuver. We also define \textit{avoid start time}, $\tsa_m$, for $\veh_m$ as:
\begin{equation}
\tsa_m  = 
\left \{ 
\begin{array}{ll}
\min_{t \in  \avoidt_{m}} t & \mbox{if~} \avoidt_{m} \neq \emptyset\\
\infty & \mbox{otherwise}
\end{array}
\right.
\end{equation}  
Therefore, $\tsa_m \in [\tsa, \tea]$ denotes the first time at which $\veh_m$ applies an avoidance maneuver and defined to be $\infty$ if $\veh_m$ never applies an avoidance maneuver. %Only one vehicle applying the avoidance maneuver at a time is thus equivalent to $\forall i \neq j \tsa_i \neq \tsa_j$ whenever . Similarly, 
Therefore, if we ensure that 
\begin{equation} \label{eqn:sep_cond}
\forall i \neq j, min(\tsa_i, \tsa_j)< \infty \implies |\tsa_i - \tsa_j| \geq \frac{\iat}{\nva} := \brd,
\end{equation}
then atmost $\nva$ vehicles are forced to apply the avoidance maneuver during the time interval $[\tsa, \tea]$. We refer to the condition in \eqref{eqn:sep_cond} as \textit{separation requirement} hereon. 

For any given time $t$, if we could find the set of all states of $\veh_i$ such that the separation requirement holds for $\veh_i$ and $\veh_m$ for all $m<i$ and for all intruder strategies, then during the path planning of $\veh_i$, we can ensure that $\veh_i$ is in one of these states at time $t$. The sequential path planning will therefore guarantee that the separation requirement holds for every SPP vehicle pair. Thus, hereon we focus on finding all states $\state_i(t)$ such that the separation requirements are ensured between vehicles $\veh_j$ and $\veh_i$, $j <i$ at time $t$ for all possible intruder scenarios (meaning all possible $\tsa, \tea, \state_{\intr}^0$ and $\ctrl_{\intr}(\cdot))$. For our analysis, we consider the following two mutually exclusive and exhaustive cases: $\infty < \tsa_j \leq \tsa_i$ and $\infty < \tsa_i < \tsa_j$. %As we will see shortly, our construction ensures that $\tsa_i \neq \tsa_j$.
In this section, we consider Case1: $\infty < \tsa_j \leq \tsa_i$. Case2 is discussed in the next section.  

In Case1, the intruder forces $\veh_j$ to apply avoidance control before or at the same time as $\veh_i$. %If $\tsa_i = \tsa_j = \infty$, then none of $\veh_i$ and $\veh_j$ need to apply avoidance control and hence trivially won't be involved in re-planning. 
To ensure the separation requirement in this case, we begin with the following two observations which narrow down the intruder scenarios that we need to consider:

\begin{observation} \label{obs1_case1}
At any time $t$, it is sufficient to consider the intruder scenarios where $\tsa \in [t-\iat, t]$. This is because if $\tsa < t - \iat$, then $\veh_i$ and/or $\veh_j$ will already be in the replanning phase at time $t$ (see assumption \ref{as:avoidOnce}) and hence we need not ensure separation requirements for them during the planning phase. On the other hand, if $\tsa > t$, then we need not ensure separation requirements at time $t$ as the intruder has not appeared in the system yet. %\SBnote{Actually, we compute obstacles at time $t'$ in a way such that their effect doesn't propagate to $t < t'$, but not sure if we need to mention this.}
\end{observation}

\begin{observation} \label{obs2_case1}
Without loss of generality, we can assume that the intruder appears at the boundary of the avoid region of $\veh_j$, e.g. $\state_{\intr, j}(\tsa) \in \partial \brs^{\text{A}}_{j}(0, \iat)$. Otherwise, vehicles need not account for the intruder until it reaches the boundary of the avoid region of $\veh_j$. Also note that since $\infty < \tsa_j \leq \tsa_i$, $\veh_{\intr}$ reaches the boundary of the avoid region of $\veh_j$ first. 
\end{observation}

==> intruder_archived_v1/intro.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\section{Response to Intruders \label{sec:intruder}}
\MCnote{Need diagrams illustrating all the different times (BRD, RD, etc.)}

\MCnote{Need to mention augmentation of static obstacles.}

In Section \ref{sec:rtt}, we presented RTT algorithm that can take into account disturbances in vehicles' dynamics. However, if a vehicle not in the set of SPP vehicles enters the system, or even worse, if this vehicle is an adversarial intruder, the original plan can lead to vehicles entering into each other's danger zones. If vehicles do not plan with an additional safety margin that takes a potential intruder into account, a vehicle trying to avoid the intruder may effectively become an intruder itself, leading to a domino effect. %In this section, we propose a method to allow vehicles to avoid an intruder while maintaining the SPP structure.

In general, the effect of an intruder on the vehicles in structured flight can be entirely unpredictable, since the intruder in principle could be adversarial in nature, and the number of intruders could be arbitrary. Therefore, we make the following two assumptions: %for our analysis to produce reasonable results, two assumptions about the intruders must be made.

\begin{assumption}
\label{as:avoidOnce}
At most one intruder (denoted as $\veh_I$ here on) affects the SPP vehicles at any given time. The intruder exits the altitude level affecting the SPP vehicles after a duration of $\iat$. 
\end{assumption}

Let the time at which intruder appears in the system be $\tsa$ and the time at which it disappears be $\tea$. Assumption \ref{as:avoidOnce} implies that $\tea \leq \tsa + \iat$. Thus, any vehicle $\veh_i$ would need to avoid the intruder $\veh_{\intr}$ for a maximum duration of $\iat$. %This assumption can be valid in situations where intruders are rare, and that some fail-safe or enforcement mechanism exists to force the intruder out of the altitude level affecting the SPP vehicles. 
Note that we do not pose any restriction on $\tsa$; however, we assume that once the intruder appears, it stays for a maximum duration of $\iat$.
%in addition, after avoiding the intruder, Qi can safely assume that it would not need to avoid another intruder

\begin{assumption}
\label{as:dynKnown}
The dynamics of the intruder are known and given by $\dot\state_\intr = f_\intr(\state_\intr, \ctrl_\intr, \dstb_\intr)$.
\end{assumption}

Assumption \ref{as:dynKnown} is required for HJ reachability analysis. In situations where the dynamics of the intruder are not known exactly, a conservative model of the intruder may be used instead. We also denote the initial state of the intruder as $\state_{\intr}^0.$ Note that $\state_{\intr}^0$ is unknown.

Our goal is to design a control policy that ensures separation with the intruder and other SPP vehicles, and ensures a successful transit to the destination. However, depending on the initial state of the intruder and its control policy, a vehicle may arrive at different states after avoiding the intruder. Therefore, a control policy that ensures a successful transit to the destination needs to account for all such possible states, which is a path planning problem with multiple initial states and a single destination, and is hard to solve in general. Thus, we divide the intruder avoidance problem into two sub-problems: (i) we first design a control policy that ensures a successful transit to the destination if no intruder appears and that successfully avoid the intruder, if it does. (ii) after the intruder disappears at $\tea$, we replan the trajectories of the affected vehicles. Following the same theme and assumptions, authors in \cite{chen2016robust} present an algorithm to avoid an intruder in SPP formulation; however, once the intruder disappears, the algorithm might need to replan the trajectories for all SPP vehicles. Since the replanning is done in real-time, it should be fast and scalable with the number of SPP vehicles, rendering the method in \cite{chen2016robust} unsuitable for practical implementation.  

In this work, we propose a novel intruder avoidance algorithm, which will need to replan trajectories only for a fixed number of vehicles, irrespective of the total number of SPP vehicles. Moreover, this number is a design parameter, which can be chosen based on the resources available during the run time. Intuitively, one can think about dividing the flight space of vehicles such that at any given time, any two vehicles are far enough from each other so that an intruder can only affect atmost $\nva$ vehicles in a duration of $\iat$ despite its best efforts. In this method, we build upon this intuition and show that such a division of space is indeed possible. The advantage of such an approach is that after the intruder disappears, we only have to replan the trajectory of \textit{atmost $\nva$} vehicles, which can be efficiently done in real-time if $\nva$ is low enough, thus making this approach particularly suitable for practical systems. %Thus the proposed method guarantees that \textit{atmost $k$} vehicles are affected by the presence of intruder, regardless of the number of SPP vehicles, and hence the replanning can be efficiently done in real-time. 

\SBnote{Fix the organization of sections once you finish writing the sections.}
In Sections \ref{sec:intruder_avoid}, we discuss the intruder avoidance control and explain the sensing range required to avoid the intruder. In Sections \ref{sec:sepRegion} and \ref{sec:buffRegion}, we compute a space division of state-space such that atmost $\nva$ vehicles need to apply the avoidance maneuver computed in Section \ref{sec:intruder_avoid}, regardless of the initial state of the intruder. However, we still need to ensure that vehicles do not collide with each other while avoiding the intruder. The induced obstacles that reflect this possibility are computed in Section \ref{sec:intruderObs}. Trajectopry planning and replanning are discussed in Sections \ref{sec:plan} and \ref{sec:replan} respectively.

==> intruder_archived_v1/plan.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Optimal Avoidance Controller} \label{sec:intruder_avoid}
Given the separation and buffer regions and induced obstacles, the overall obstacle for $\veh_i$ is given by:
\begin{equation}
\label{eq:obsseti_intr}
\obsset_i(t)  = \soset_i \cup \bigcup_{j=1}^{i-1} \left( \tilde{\buff}_{ij}(t) \cup \tilde{\buff}_{ji}(t) \cup_{k=1}^{5} {^k\ioset_i^j}(t) \right)
\end{equation}

Given $\obsset_i(t)$, we compute a BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ for path planning that contains the initial state of $\veh_i$ while avoiding these obstacles:
\begin{equation} \label{eqn:intrBRS1}
\begin{aligned}
\brs^{\text{AO}}_{i}(t, \sta_i) = & \{y: \exists \ctrl_i(\cdot) \in \cfset_i, \forall \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \forall s \in [t, \sta_i], \state_i(s) \notin \obsset_i(s), \\
& \exists s \in [t, \sta_i], \state_i(s) \in \targetset_i, \state_i(t) = y \}.
\end{aligned}
\end{equation}
The Hamiltonian $\ham^{\text{AO}}_{i}$ to compute BRS in \eqref{eqn:intrBRS1} is given by:
\begin{equation} \label{eqn:BRSham}
\ham^{\text{AO}}_{i}(\state_i, \costate) = \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}

Note that $\brs^{\text{AO}}_{i}(\cdot)$ ensures goal satisfaction for $\veh_i$ in the absence of intruder. The goal satisfaction controller is given by:
\begin{equation}
{\ctrl^{\text{AO}}_{i}}(t, \state_i) = \arg \min_{\ctrl_i \in \cset_i} \max_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{equation}
Moreover, if $\veh_i$ starts within $\brs^{\text{AO}}_{i}$, it is guaranteed to avoid collision with other vehicles for a duration of $\iat$, starting at any $\tsa < \sta_i$, irrespective of the control and disturbance applied by vehicles (including $\veh_i$ itself) during this time period. 

\begin{remark}
Note that if we use the robust trajectory tracking method to compute the base obstacles, we would need to augment the obstacles in \eqref{eq:obsseti_intr} by the error bound of $\veh_i$, $\disckernel_i$, as discussed in section \ref{sec:rtt}.
\end{remark}

To compute the optimal avoidance control for $\veh_i$ in presence of $\veh_{\intr}$, we compute the set of states from which the joint states of $\veh_{\intr}$ and $\veh_i$ can enter danger zone $\dz_{i\intr}$ despite the best efforts of $\veh_i$ to avoid $\veh_{\intr}$. Given the relative dynamics in \eqref{eq:reldyn}, this set of states is given by the BRS $\brs^{\text{S}}_{i}(\tau, \iat),~ \tau \in [0, \iat]$, given by \eqref{eqn:sepBRS}.

Once the value function $\valfunc^{\text{S}}_{i}(\cdot)$ is computed, the optimal avoidance control ${\ctrl^{\text{S}}_{i}}$ can be obtained as:
\begin{equation} \label{eqn:optAvoidCtrl}
{\ctrl^{\text{S}}_{i}} = \arg \max_{\ctrl_i \in \cset_i} \left( \min_{\ctrl_\intr \in \cset_\intr, \dstb_i \in \dset_i, \dstb_\intr \in \dset_\intr} \costate \cdot f_r(\state_{\intr, i}, \ctrl_i, \ctrl_\intr, \dstb_i, \dstb_\intr) \right)
\end{equation}

Under normal circumstances when the intruder $\veh_{\intr}$ is far away, we have $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) > 0$; as $\veh_{\intr}$ gets closer to $\veh_i$, $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t))$ decreases. If $\veh_i$ applies the control ${\ctrl^{\text{S}}_{i}}$ when $\valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) = 0$, then collision avoidance between $\veh_i$ and $\veh_{\intr}$ is guaranteed for a duration of $\iat$ under the worst-case intruder control strategy $\ctrl_\intr$.

In addition, computation of $\obsset_i(\cdot)$ ensures that $\veh_i$ does not collide with any other SPP vehicle during the avoidance maneuver. %Therefore, applying $\ctrl_I^A$ for a duration of $\iat$ is still guaranteed to keep $\veh_i$ safe from all obstacles, and hence safe from collision with respect to all other vehicles $\veh_j, j \neq i$.
The overall control policy for avoiding the intruder and collision with other vehicles is thus given by:
\begin{equation*}
{\ctrl^{\text{A}}_{i}}(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{AO}}_{i}}(t) & t \leq \tsa\\
{\ctrl^{\text{S}}_{i}}(t) & \tsa\leq t \leq \tea
\end{array}
\right.
\end{equation*}

\SBnote{Somewhere mention the conditions under which our method is guaranteed to avoid the intruder.} 

==> intruder_archived_v1/replan.tex <==
% !TEX root = ../SPP_IoTjournal.tex
\subsection{Replanning after intruder avoidance} \label{sec:replan}
Intruder can force some SPP vehicles to deviate from their planned trajectory; therefore, we have to replan the trajectory of these vehicles once $\veh_{intr}$ disappears. The set of all vehicles $\veh_i$ for whom we need to replan the trajectories, $\rvs$, can be obtained by checking if a vehicle $\veh_i$ applied any avoidnace control during $[\tsa, \tea]$, e.g.,
\begin{equation} \label{eq:RVS}
\rvs = \{\veh_i, i \in \{1, \ldots, \N \}: \valfunc^{\text{S}}_{i}(0, \state_{\intr, i}(t)) \leq 0, t \in [\tsa, \tea] \}. 
\end{equation}  

Note that due to the presence of separation and buffer regions, atmost $\nva$ vehicles can be affected by $\veh_{intr}$, e.g. $|\rvs| \leq \nva$. Goal satisfaction controllers which ensure that these vehicles reach their destinations can be obtained by solving a new SPP problem, where the starting states of the vehicles are now given by the states they end up in, denoted $\tilde{\state}_i^0$, after avoiding the intruder. Let the optimal control policy corresponding to this liveness controller be denoted ${\ctrl^{\text{L}}_{i}}(t, \state_i)$. The overall control policy that ensures intruder avoidance, collision avoidance with other vehicles, and successful transition to the destination for vehicles in $\rvs$ is given by:

\begin{equation*}
\ctrl_i^*(t) = 
\left \{ 
\begin{array}{ll}
{\ctrl^{\text{A}}_{i}}(t, \state_i) & t \leq \tea\\
{\ctrl^{\text{L}}_{i}}(t, \state_i) & t > \tea
\end{array}
\right.
\end{equation*}

Note that in order to re-plan using a SPP method, we need to determine feasible $\sta_i$ for all vehicles. This can be done by computing an FRS:
\begin{equation} \label{eq:re-planFRS}
\begin{aligned} 
\frs_i^{\text{RP}}(\tea, t) = & \{y \in \R^{n_i}: \exists \ctrl_i(\cdot) \in \cfset_i, \forall \dstb_i(\cdot) \in \dfset_i, \\
& \state_i(\cdot) \text{ satisfies \eqref{eq:dyn}}, \state_i(\tea) = \tilde{\state}_i^0, \\
& \state_i(t) = y, \forall s \in [\tea, t], \state_i(s) \notin \obsset_i^{\text{RP}}(s) \},
\end{aligned}
\end{equation}
\noindent where $\tilde{\state}_i^0$ represents the state of $\veh_i$ at $t = \tea$; $\obsset_i^{\text{RP}}(\cdot)$ takes into account the fact that $\veh_i$ needs to avoid higher-priority vehicles $\veh_j, j<i$ and is defined in an way analogous to \eqref{eq:obsseti}.
%\begin{equation} 
%\obsset_j^{\text{RP}}(t) = \bigcup_{k<j} \frs_k^{\text{RP}}(\tea, t), ~~~t > \tea.
%\end{equation}

The FRS in \eqref{eq:re-planFRS} can be obtained by solving %the HJ VI in \eqref{eq:HJIVI_FRS} with the following Hamiltonian:

\begin{equation}
\begin{aligned}
\max \Big\{&D_t \valfuncfwd_i^{\text{RP}}(t, \state_i) + \ham_i^{\text{RP}}(t, \state_i, \nabla \valfuncfwd_i^{\text{RP}}(t, \state_i)), \\
&\qquad - \obsfunc_i^{\text{RP}}(t, \state_i) - \valfuncfwd_i^{\text{RP}}(t, \state_i) \Big\} = 0\\
&\valfuncfwd_i^{\text{RP}}(\tsa, \state_i) = \max\{\fc_i^{\text{RP}}(\state_i), -\obsfunc_i^{\text{RP}}(\tsa, \state_i)\} \\
&\ham_i^{\text{RP}}(\state_i, \costate) = \max_{\ctrl_i \in \cset_i} \min_{\dstb_i \in \dset_i} \costate \cdot f_i (\state_i, \ctrl_i, \dstb_i)
\end{aligned}
\end{equation} 

\noindent where $\valfuncfwd_i^{\text{RP}}, \obsfunc_i^{\text{RP}}, \fc_i^{\text{RP}}$ represent the FRS, obstacles during re-planning, and the initial state of $\veh_i$, respectively. The new $\sta$ of $\veh_i$ is now given by the earliest time at which $\frs_i^{\text{RP}}(\tea, t)$ intersects the target set $\targetset_i$, $\sta_i := \arg \inf_t \{ \frs_i^{\text{RP}}(\tea, t) \cap \targetset_i \neq \emptyset \}$. Intuitively, this means that there exists a control policy which will steer the vehicle $\veh_i$ to its destination by that time, despite the worst case disturbance it might experience.

\begin{remark}
Note that even though we have presented the analysis for one intruder, the proposed method can handle multiple intruders as long as only one intruder is present \textit{at any given time}. 
\end{remark}

We conclude this section with the overall SPP algorithm that takes into account an intruder that may appear for a duration of $\iat$: 
\begin{alg}
\label{alg:intruder}
\textbf{Intruder Avoidance algorithm (offline planning)}: Given initial conditions $\state_i^0$, vehicle dynamics \eqref{eq:dyn}, intruder dynamics in Assumption \ref{as:dynKnown}, target sets $\targetset_i$, and static obstacles $\soset_i, i = 1\ldots, \N$, for each $i$,
\begin{enumerate}
\item determine the separation region and buffer regions given by \eqref{eqn:sepRegion}, \eqref{eqn:augbuffRegion1} and \eqref{eqn:augbuffRegion2}.
\item compute the induced obstacles for $\veh_i$ by $\veh_j$ given by \eqref{eq:intruderObs_case1}, \eqref{eq:intruderObs_case2}, \eqref{eq:intruderObs_case3}, \eqref{eq:intruderObs_case4} and \eqref{eq:intruderObs_case5}. 
\item compute the total obstacle set $\obsset_i(t)$, given in \eqref{eq:obsseti_intr}. In the case $i=1$, $\obsset_i(t) = \soset_i ~ \forall t$;
\item given $\tilde\obsset_i(t)$, compute the BRS $\brs^{\text{AO}}_{i}(t, \sta_i)$ defined in \eqref{eqn:intrBRS1};
\item the optimal control to avoid the intruder can be obtained by using \eqref{eqn:optAvoidCtrl};
\end{enumerate}

\textbf{Intruder Avoidance algorithm (online re-planning)}: For each vehicle $\veh_i \in \rvs$ which performed avoidance in response to the intruder,
\begin{enumerate}
\item compute $\frs_i^{\text{RP}}(\tea, t)$ using $\eqref{eq:re-planFRS}$. The new $\sta_i$ for $\veh_i$ is given by $\arg \inf_t \{ \frs_j^{\text{RP}}(\tea, t) \cap \targetset_j \neq \emptyset \}$;
\item given $\sta_i$, $\tilde{\state}_i^0$, vehicle dynamics \eqref{eq:dyn}, target set $\targetset_i$, and obstacles $\obsset_i^{\text{RP}}$, use any of the three SPP methods discussed in \cite{chen2016robust} for re-planning. 
\end{enumerate}
\end{alg}
